Keeping up with "The Joneses": reference dependent choice with social comparisons

Keeping up with "The Joneses" matters. This paper examines a model of reference dependent choice where reference points are determined by social comparisons. An increase in the strength of social comparisons, even by only a few agents, increases consumption and decreases welfare for everyone. Strikingly, a higher marginal cost of consumption can increase welfare. In a labour market, social comparisons with co-workers create a big fish in a small pond effect, inducing incomplete labour market sorting. Further, it is the skilled workers with the weakest social networks who are induced to give up income to become the big fish.

==> 3.labour_market.tex <==
The previous section explored the effects of social comparisons on consumption decisions, without taking a view as to exactly what it is that agents consume. Here, I move to looking at agents' firm choices in the labour market in order to explore labour market \emph{sorting} and \emph{segregation}.\footnote{Sorting is where skilled workers work (disproportionately) for high-productivity firms. Segregation is where skilled workers work (disproportionately) with each other.} 
To do this, I extend the model to a setting where agents make social comparisons with both their neighbours (as in the previous section) and also their \emph{co-workers}. For tractability, I do not model an explicit social network within a firm -- agents compare themselves to the simple average within their firm.

I find that stronger social comparisons with co-workers reduces labour market sorting and segregation, total output, and also income inequality. Additionally, welfare of all skilled is decreasing in the strength of these social comparisons and the skilled workers with the weakest social comparisons with friends are the ones who work for the low productivity firms and so earn lower wages.


\subsection{Model}
\textbf{Types.} There are two types of workers: \emph{skilled} and \emph{unskilled}, with ability $e_S$ and $e_U$ respectively. There are two types of firms: \emph{high productivity} and \emph{low productivity}, with productivity $k_H$ and $k_L$ respectively. Assume each firm has a fixed, but large, number of vacancies (this allows a firm to have any fraction of skilled workers and simplifies the analysis). Denote typical workers $i,j$, and firm $m$. W.L.O.G. let $e_U \equiv 1$ and $k_L \equiv 1$. To keep things clear, assume that half of workers are skilled, half of firms are high productivity, and the number of workers equals the number of vacancies (so there will be no unemployment in this model). \\

\noindent \textbf{Jobs.}
Workers $i$ and firms $m$ match to form \emph{jobs}. When they do, the total surplus of a job is $y_{im} = e_i k_m$.  A firm and worker bargain over this surplus. If they do not agree on a split, both receive zero. %This is because neither a firm nor a worker can generate any surplus outside of a job. 
The worker's wage is therefore a fraction, $\gamma$, of the surplus. So when worker $i$ works at firm $m$: $w_{i} = \gamma y_{im}$. This is the standard axiomatic bargaining outcome.
Any worker $i$ can apply to any firm $m$. If a firm $m$ receives more applications than it has vacancies, then it chooses workers to maximise its own pay-off, and randomise when indifferent.\footnote{Due to the assumption about the match surplus, firms will always choose skilled workers over unskilled workers. Firms also choose at random between different skilled workers and between different unskilled workers.}

Skilled workers and high productivity firms both have an outside option during the bargaining process. Skilled workers can work for either type of firm, and high productivity firms can employ either type of worker. However, these outside options are worse than the standard bargaining outcome without an outside option, and so have no impact on the outcome \citep[Proposition 6]{binmore1986nash}. \\

\noindent \textbf{Social comparisons.} An agent's reference point is a now weighted average of her \emph{friends'} wage \emph{plus} a simple average of her \emph{co-workers'} wage. Co-workers are other agents that work at the same firm. Therefore, part of her reference point is (endogenously) determined by her choice of job.

Assume that $\alpha = \alpha_{1i} + \alpha_{2i}$, \emph{the overall strength of social comparisons}, is identical for all agents. Then $\alpha_{1i} = \sum_j G_{ij}$. Therefore $\alpha_{2i}$ is a residual term. Also assume that $\alpha_{1i} \leq \alpha$ for all $i$, and (to guarantee existence) $\alpha < 1$.
This yields:
\begin{align*}
	u_i = f(w_{i} - \alpha_{1i} \sum_{j} g_{ij} w_{j} - \alpha_{2i} \gamma \overline{w}_m) + b \sum_j \alpha_{1i} g_{ij}
\end{align*}
where $\overline{w}_m$ is the average wage at firm $m$. For tractability purposes, assume that there is not exactly one agent of any given type and that the linking benefit parameter, $b$, is common to all agents.


\subsection{Results}
Armed with the model, we can now examine how social comparisons determines workers' \emph{sorting} into firms. First, it is helpful to present a very simple definition of labour market sorting.

\begin{defn}[Sorting]\label{defn:sorting}
	Sorting is equal to the fraction of skilled workers that work for high productivity firms, $c$.
\end{defn}

Sorting captures the extent to which workers and firms match along lines of skill and productivity. Absolute deviations of $c$ from $\frac{1}{2}$ capture segregation -- the extent to which workers are concentrated in firms with other workers of the same type. Skilled workers will never disproportionately concentrate in low productivity firms, so in practice the two definitions coincide, and it suffices to simply consider $c$.

\begin{rem}\label{rem:disproportionate skilled}
	Skilled workers work disproportionately for high productivity firms. Formally: $c^* > \frac{1}{2}$.
\end{rem}

This is because the only incentive for a skilled worker to choose a low productivity firm is to reduce her reference point by having lower-earning co-workers. If skilled workers worked disproportionately for low productivity firms, then this incentive would not be present. The key insight in this section is that social comparisons with co-workers \emph{induce} less labour market sorting. %, and that this relationship is monotonic.

\begin{prop}[Sorting]\label{prop:sorting}
	If the strength of social comparisons with co-workers weakly increases for all workers, then labour market sorting weakly decreases.
\end{prop}

Social comparisons with co-workers can cause a skilled worker to choose to work for low productivity firms because they want to be a \emph{``big fish in a small pond''}. This is because average wages are lower at low productivity firms, and having lower co-worker wages reduces her reference point. When comparisons with co-workers are strong enough the benefit of improving her wage \emph{relative to her co-workers} outweighs the cost of a lower \emph{absolute} wage. If social comparisons with co-workers become stronger, then the ``big fish'' effect becomes more prominent, so skilled workers may shift to low productivity firms.%\footnote{This increases average wages at low productivity firms (and reduces them at high productivity firms), reducing the incentive for further skilled workers to shift to low productivity firms. Hence we get a shift to a new equilibrium, rather than a mass exodus.} 

Notice that the structure of the social network (of friends) does not play a direct role here. This is because it, and friends' wages, do not change in response to a worker's choice of firm. In contrast, the \emph{strength} of social comparisons with friends does matter, because of the assumption that total weight a workers places of social comparisons is fixed. This means that stronger comparisons with friends causes weaker comparisons with co-workers. Intuitively, we can think of the total strength of social comparisons as determined separately from the relative weight put on friends versus co-workers. Consequently, outcomes for skilled workers -- where they work and how much they earn -- are intimately tied to their social networks. 

\begin{prop}\label{prop:network sorting}
There exists a threshold value $\alpha_1^{crit}$ such that a skilled worker works at a high productivity firm if and only if $\alpha_{1i} \geq \alpha_1^{crit}$.
\end{prop}

This means that all skilled workers at high productivity firms make stronger social comparisons with friends than all skilled workers at low productivity firms. Those with the strongest social comparisons with friends experience the weakest desire to be a ``big fish in a small pond'', and so choose to work for high productivity firms. 

The result in fact gives us a complete characterisation of which type of firm every skilled worker chooses. A fraction $c$ of skilled workers work at high productivity firms. These are precisely the fraction $c$ of skilled workers with the highest weighted degree. The result does not extend to unskilled workers because unskilled workers are forced to take whatever vacancies are left over, and firms are indifferent between all unskilled workers. Now that we know who works where (at least among skilled workers) and how this depends on social comparisons, we can examine how the strength of social comparisons affects wages at the individual level.

\begin{cor}\label{cor:network sorting}
    For a skilled worker, stronger social comparisons with friends weakly increases her wage.
    %There exists a threshold value $\alpha^{crit}$, such that all skilled workers with a strength of social comparisons with friends above this threshold earn more than all skilled workers below the threshold.
	%Skilled workers at high productivity firms make stronger social comparisons with their friends than skilled workers at low productivity firms.
\end{cor}

This happens because stronger social comparisons with friends reduces the strength of social comparisons with co-workers. So the ``big fish'' effect is weaker, and she cares more about her absolute wage. She may then switch from a low productivity firm (with lower wages) to a high productivity firm (with higher wages). In this simple setting with only two types of firms, she will switch when her strength of social comparisons with friends passes a threshold.

Having examined how social comparisons affect labour market sorting, it is natural to consider the role of skill and productivity. The effects are highly intuitive. 

\begin{rem}[Comparative statics]\label{rem:comparative statics}
	The extent of labour market sorting is weakly monotonically increasing in the productivity of high productivity firms, $k_H$, and is weakly monotonically decreasing ability of skilled workers, $e_S$.
\end{rem}

When $k_H$ rises, the foregone wage from choosing to work at a low productivity firm is larger. This makes working at low productivity firms less attractive, so skilled workers do it less. Conversely, when $e_H$ rises, then the ``big fish'' effect becomes more prominent, as skilled workers earn more relative to their unskilled co-workers. This makes low productivity firms more attractive to skilled workers. Finally, I turn to three key outcomes of the model: output, inequality, and welfare. 

\begin{prop}\label{prop:output,var,welfare}
    An increase in the overall strength of social comparisons, $\alpha$: \\
    (i) weakly reduces output, \\
    (ii) weakly reduces the variance in wages, \\
    (iii) weakly reduces welfare of every skilled worker.
\end{prop}

The output and variance results follow from the complementarity of worker skills and firm productivity.  Social comparisons drive the extent of labour market sorting. In turn, more sorting increases total output, and makes it more unequally spread. The variance result does not extend to standard measure of inequality, such as the Gini coefficient, because the strength of social comparisons affect the average wage. Decreased sorting induced by stronger social comparisons moves workers from the extremes towards the centre, which reduces inequality. However, the fall in the average wage can more than offset this. The welfare result is analogous to \Cref{prop:ref strength}. Stronger social comparisons reduce a skilled worker's wage \emph{relative to} her reference point. \\

\noindent \textbf{Social network formation.} Allowing agents to choose their links in the main model led to a set of ``social classes''. Each ``social class'' differed in their level of consumption and Bonacich centrality. It is natural to extend this analysis to the case with a labour market. I first consider how links with friends form when the overall strengths of social comparisons with friends and co-workers are fixed. This holds the density of friendships constant and examines the resulting pattern. 

As before, I assume that links are symmetric, and allow agents to propose any links they like. Further, links require mutual consent to form and can be broken unilaterally. I then look for pairwise stable networks (see page 11 for a definition). This process of endogenous network formation leads to agents segregating based on income.

\begin{prop}\label{prop:labour endo network}
    Fix $\alpha_{1i}$ and $\alpha_{2i}$ for all $i$. In all pairwise stable networks, $g_{ij} > 0$ only if $w_i = w_j$.
\end{prop}


Agents only form links with others who have the same level of income. This means that agents segregate into ``social classes'' where everyone has the same level of skill \emph{and} works for the same type of firm.\footnote{In the special case where $e_S = k_H$ then skilled workers at low productivity firms and unskilled workers at high productivity firms share a social class. However, this is a knife edge case.}
%These social classes are not only based on both agents' innate characteristics (their skill), but also their decisions in the labour market (the type of firm they work for). 
This strongly contrasts with \Cref{prop:network sorting}. Social comparisons with co-workers can reduce sorting in the labour market, but cause extreme social sorting in friendship networks.

Intuitively, everyone would like to have friends with lower income than themselves, so they can feel like they are ahead of ``The Joneses''. However, friendships require mutual consent. So no agent wants to become friends with someone who has higher income -- as doing so would generate unfavourable social comparisons. As a consequence, agents only become friends with people similar to themselves (in terms of income).


\subsection{Discussion}

%\textbf{The sorting puzzle.} 
\cite{song2019firming} find that the majority of the increase in inequality in the US over the past 40 years is due to increased sorting and segregation in labour markets.\footnote{\cite{song2019firming} use a confidential database from the U.S. Social Security Administration, which contains earnings records for every individual ever issued a U.S. Social Security number. Earnings data are uncapped and contain all sources of income deemed as remuneration by the U.S. Internal Revenue Service. They use the full dataset from 1981 to 2013.}
Their analysis raises two questions. Why didn't skilled workers sort into high productivity firms and only work with similarly-skilled peers in the first place? And what caused sorting and segregation to increase? Rising returns to skills -- a common explanation for rising inequality -- would mechanically increase sorting and segregation, but \citet[p38]{song2019firming} show that this can only explain a (small) minority of the changes.

Social comparisons with co-workers provide a possible answer to both of these questions. First, the presence of social comparisons leads to skilled workers not sorting in the first place. Second, changes to the relative importance of friends versus co-workers as the source of social comparisons can explain the increase in sorting over time. This could have been caused by the rapid growth in social media use over recent decades.  In 2021, 72\% of Americans use at least one social platform, up from only 5\% in 2005 [Pew Research Center, \citeyear{pew2021social}]. This has made it easier to maintain relationships with your friends \citep{liu2016meta, ellison2007social} observe the your friends' consumption, and compare yourself to them \citep{verduyn2017social}.

In contrast, there has been no change of comparable magnitude to the ways in which we can compare ourselves to our co-workers. I contend that these changes to technology over recent decades have increased the extent to which people make social comparisons with their friends, relative to those they make with their co-workers. This provides an explanation for the increased sorting observed by \cite{song2019firming}.

%\textbf{Social networks and wages.} 
Separate to the \emph{extent} of sorting, the results concerning \emph{who works where} provide a new mechanism through which social networks affect labour market outcomes. In this paper, skilled workers choose high wage jobs because the pressure from their social network to earn more outweighs their desire to be the ``big fish'' in the workplace. Social networks do not help skilled agents obtain high wage jobs that they would be otherwise unable to get. Rather the social comparisons pressure skilled agents into high wage jobs they would not otherwise choose. This provides a contrasting view to the existing literature, which suggests that strong social networks can increase earnings by improving agents' opportunities or productivity. For example, strong social networks provide improved access to job information \citep{ioannides2004job}, or referrals from existing employees \citep{montgomery1991social}.

In my set-up, the skilled workers who end up at the lower productivity, lower paying, firms do so because they choose to. They are not held back by a lack of ability or insider access. Rather, they have relatively weak social networks, and so care a lot about their co-workers. It is their preferences that drive them to earning lower wages. The implications for policy-makers are mixed. On the one hand, giving (currently) poorer skilled agents stronger social networks can increase their earnings. However, this requires changing these agents' preferences, and leaves them with lower utility.

%\textbf{Further applications.} 
%The extended model we present in this section could also be applied to spatial choice, where an both agent's consumption and her immediate neighbours (and their consumption) depends on her choice of location. For example, we could think about choosing a street to live on. A street provides consumption of local amenities, such as beautiful parks, good access to public transport, and crime-free streets. It also brings a set of neighbours, who also have similar access to these local amenities. However it does not affect her friends' consumption -- the local amenities where they live remain the same when the agent moves into a new street. More generally, we could equally apply it to any situation where the choice an agent makes affects her consumption and the consumption of some people she must interact with (as a result of that choice), but \emph{does not} affect her friends. 



==> A2.proofs_applications.tex <==
% COMMENT: WE NEED TO PROVE PROPOSITION ON FIRM CHOICE BEFORE PROVING THE REMARK ON MINIMUM SORTING
\noindent The simplest proof to Remark \ref{rem:disproportionate skilled} relies on Proposition \ref{prop:sorting} and Remark \ref{rem:comparative statics}, so we defer the proof until after Remark \ref{rem:comparative statics}. It is also more convenient to express wages, $w_{im}$, as $\gamma e_i k_m$.

% ------------------------------------------------------------- %
% PROVES THAT STRONGER SOCIAL COMPARISONS WEAKLY DECREASE SORTING
% ------------------------------------------------------------- %
\begin{proof}[\emph{\textbf{Proof of \Cref{prop:sorting}.}}]
	\textbf{Firm choice.} Firms always choose skilled workers over unskilled workers (by assumption), so it suffices to consider where the skilled workers choose to work. Unskilled workers fill up all remaining vacancies (since we have assumed that there are as many vacancies as workers). A skilled worker $i$ will apply for a job at a high productivity firm only if and only if:
	\begin{align}
		f(\gamma e_S k_H - \alpha_{1i} \sum_{l} g_{il} \gamma e_{l} k_{l} - \alpha_{2i} \gamma \overline{e}_{H} k_H) &\geq f(\gamma e_S - \alpha_{1i} \sum_{l} g_{il} \gamma e_{l} k_{l} - \alpha_{2i} \gamma \overline{e}_{L})
	\end{align}
	Simplifying and rearranging yields $\frac{1}{\alpha_{2i}} e_S (k_H - 1) \geq k_H \overline{e}_H - \overline{e}_L$. By definition: $\frac{1}{2}( e_S + 1) = \overline{e} = \frac{1}{2}(\overline{e}_H + \overline{e}_L)$, where $\overline{e}$ is the global average skill. Substituting out $\overline{e}_{L}$: $\frac{1}{\alpha_2} e_S (k_H - 1) \geq (1 + k_H) \overline{e}_H - e_S - 1$. Let $c$ be the fraction of skilled workers working for at high productivity firms. Then $\overline{e}_H = c e_S + (1-c) = 1 + c(e_S - 1)$. Substituting in for $c$ yields:
	\begin{align}\label{eq:firm choice ineq}
		\frac{1}{\alpha_{2i}} e_S (k_H - 1) \geq (1 + k_H) [1 + c(e_S - 1)] - e_S - 1
	\end{align}
	For any $c$ there exists a critical value of $\alpha_{2i}$ such that equation \ref{eq:firm choice ineq} holds with equality (i.e. skilled worker $i$ is indifferent between working at a high productivity and low productivity firm). Denote this value $\alpha_{2i}^{crit}$. This follows from the fact that that the Left-Hand Side (LHS) is decreasing in $\alpha_{2i}$, while the Right-Hand Side (RHS) does not depend on $\alpha_{2i}$. LHS of equation \ref{eq:firm choice ineq} is strictly decreasing in $c$, while RHS does not depend on $c$. So $\alpha_{2i}^{crit}$ is a strictly decreasing function of $c$. Denote this function $\alpha_{2i}^{crit} = h(c)$, with $h'(c) < 0$.

	\textbf{Existence.} Let $F(\cdot)$ denote the C.D.F. of $\alpha_{2i}$ (i.e. the fraction of skilled workers with an $\alpha_{2i}$ value of less than or equal to $\alpha_2$). Therefore $F(h(c))$ is the fraction of skilled workers who want to work at high productivity firms, given that a fraction $c$ of skilled workers actually work at high productivity firms. An equilibrium is then a fixed point of this equation:  $F(h(c)) = c$. RHS of this is strictly increasing in $c$, and LHS is weakly decreasing in $c$, so there exists a fixed point, $c^*$.

	\textbf{Monotonicity.} Suppose that $\alpha_{2i}$ weakly increases for all $i$. Then $F(a)$ weakly decreases for all $a$ (this follows from well-known properties of C.D.F.s). This in turn reduces $F(h(c))$ for any $h(c)$, which weakly reduces $c^*$. Notice that $F(h(c)) = 1$ for all values of $c$ where $h(c) \geq \max_{i} \alpha_{2i}$.
\end{proof}
% ------------------------------------------------------------- %




% ------------------------------------------------------------- %
% PROVES THAT SKILLED WORKERS WITH HIGH DEGREE CENTRALITY WORK AT HIGH PRODUCTIVITY FIRMS
% ------------------------------------------------------------- %
\begin{proof}[\emph{\textbf{Proof of \Cref{prop:network sorting}.}}]
	From \Cref{prop:sorting}, for any $c$, there exists an agent-specific critical value $\alpha_{2i}^{crit}$ such that: \textbf{(a)} when $\alpha_{2i} = \alpha_{2i}^{crit}$, $i$ is \emph{indifferent} between high productivity and low productivity firms, \textbf{(b)} when $\alpha_{2i} < \alpha_{2i}^{crit}$, $i$ strictly prefers a \emph{high} productivity firm, \textbf{(c)} when $\alpha_{2i} > \alpha_{2i}^{crit}$, $i$ strictly prefers a \emph{low} productivity firm. \Cref{prop:sorting} also proved that there exists some equilibrium level of labour market sorting, $c^*$. 
	
	This yields an equilibrium critical value for $\alpha_{2}$. Denote it $\alpha_{2,eq}^{crit}$. Therefore, all skilled workers with $\alpha_{2i} \leq \alpha_{2,eq}^{crit}$ work at high productivity firms. All skilled workers with  $\alpha_{2i} \geq \alpha_{2,eq}^{crit}$ work at low productivity firms. 
	Finally, notice that $\alpha = \alpha_{1i} + \alpha_{2i}$ (by assumption), so a threshold in $\alpha_2$ is easily converted to a theshold in $\alpha_1$. %and that $\alpha_{1i}$ captures the strength of $i$'s comparisons with her friends (by definition). Therefore higher $\alpha_{1i}$ implies lower $\alpha_{2i}$.
\end{proof}
% ------------------------------------------------------------- %

\begin{proof}[\emph{\textbf{Proof of \Cref{prop:network sorting}.}}]
This follows straightforwardly from \Cref{prop:network sorting}. An increase in the strength of social comparisons for a skilled worker (i.e. an increase in $\alpha_{1i}$ causes a decrease in $\alpha_{2i}$. This either moves the agent to the other side of the threshold (in $\alpha_2$), or it does not. In the first case, she moves to the low productivity firm and her wage falls. In the second case, she stays at the same firm, and her wage remains unchanged.
\end{proof}


% ------------------------------------------------------------- %
% PROVES THE COMPARATIVE STATICS FOR E_H AND K_H
% ------------------------------------------------------------- %
\begin{proof}[\emph{\textbf{Proof of \Cref{rem:comparative statics}.}}]
    \Cref{prop:sorting} found a critical value $\alpha_{2,eq}^{crit}$ such that \cref{eq:firm choice ineq} holds with equality. Rearranging \cref{eq:firm choice ineq} in this case yields:
	$$c^* = (e_S - 1)^{-1} (k_H + 1)^{-1} \left( \frac{1}{ \alpha_{2,eq}^{crit} } e_S (k_H - 1) + e_S - k_H \right)$$
    Suppose there is an interior solution: $c^* \in (0,1)$. Then $\alpha_{2,eq}^{crit} < \max_i \alpha_{2i}$ (otherwise no skilled workers would choose a high productivity firms). Since $\alpha_{1i} + \alpha_{2i} = \alpha < 1$ (by assumption), then $\alpha_{2,eq}^{crit} < 1$.  By standard rules of differentiation, and rearranging terms:
	\begin{align*}
		%c &= (e_S - 1)^{-1} (k_H + 1)^{-1} \left( \frac{1}{\alpha_2} e_S (k_H - 1 + \alpha_{2}) - k_H \right) \\
		%\frac{d c}{d e_S} &= (-1)(e_S - 1)^{-2} (k_H + 1)^{-1} \left( \frac{1}{\alpha_2} e_S (k_H - 1) + e_S - k_H \right)
		%+ (e_S - 1)^{-1} (k_H + 1)^{-1} \frac{1}{\alpha_2} (k_H - 1 + \alpha_{2}) \\
		%&= (e_S - 1)^{-2} (k_H + 1)^{-1}  \frac{1}{\alpha_2}  \left( - e_S (k_H - 1) - \alpha_{2} e_S + \alpha_{2} k_H + (e_S -1) (k_H - 1 + \alpha_{2}) \right)	\\
		%&= (e_S - 1)^{-2} (k_H + 1)^{-1}  \frac{1}{\alpha_2}  \left( -(k_H - 1 + \alpha_{2}) + \alpha_{2} k_H    \right) \\
		\frac{d c^*}{d e_S} = \frac{(\alpha_{2,eq}^{crit} - 1)(k_H - 1)}{\alpha_2  (e_S - 1)^{2} (k_H + 1)} \quad < 0 
		\qquad \text{and} \qquad 
		%\frac{d c}{d e_S} &< 0
		\frac{d c^*}{d k_H} = \frac{e_S (2 - \alpha_{2,eq}^{crit}) - \alpha_{2,eq}^{crit} }{ \alpha_{2,eq}^{crit} (k_H + 1)^{2}} \quad > 0  %\\
	\end{align*}
    Since $e_S > 1$, $k_H > 1$, $\alpha_{2,eq}^{crit} < 1$. If instead there is a corner solution, then $\frac{d c^*}{d e_S} = 0$ and $\frac{d c^*}{d k_H} = 0$.
	%\begin{align*}
		%c &=  (e_S - 1)^{-1} (k_H + 1)^{-1} \left( k_H (\frac{1}{\alpha_2} e_S - 1) + e_S(1 - \frac{1}{\alpha_{2}}) \right) \\
		%\frac{d c}{d k_H} &= (-1)(e_S - 1)^{-1} (k_H + 1)^{-2} \left( k_H (\frac{1}{\alpha_2} e_S - 1) + e_S(1 - \frac{1}{\alpha_{2}}) \right)
		%+ (e_S - 1)^{-1} (k_H + 1)^{-1} (\frac{1}{\alpha_2} e_S - 1) \\
		%&= (e_S - 1)^{-1} (k_H + 1)^{-2} \left( -k_H (\frac{1}{\alpha_2} e_S - 1) - e_S(1 - \frac{1}{\alpha_{2}}) + (k_H + 1)(\frac{1}{\alpha_2} e_S - 1)   \right)  \\
		%&= (e_S - 1)^{-1} (k_H + 1)^{-2} \left( (\frac{1}{\alpha_2} e_S - 1) - e_S(1 - \frac{1}{\alpha_{2}})  \right) \\
		%\frac{d c}{d k_H} &= \frac{e_S (2 - \alpha_{2}) - \alpha_{2}}{\alpha_{2} (k_H + 1)^{2}} \quad > 0  \\
		%&> 0
	%\end{align*}
	%Since $c^* = c$ if $c \in [0,1]$ and $c^* = 1$ if $c >1$, then $\frac{d c^*}{d e_S} \leq 0$ and $\frac{d c^*}{d k_H} \geq 0$.
\end{proof}
% ------------------------------------------------------------- %



% ------------------------------------------------------------- %
% PROVES THAT SORTING (C) IS ALWAYS LARGER THAN 0.5
% ------------------------------------------------------------- %
\begin{proof}[\emph{\textbf{Proof of \Cref{rem:disproportionate skilled}.}}]
	$c^*$ is weakly monotonically decreasing in $\alpha$ (\Cref{prop:sorting}). $c^*$ is weakly monotonically decreasing in $e_S$, and weakly monotonically increasing in $k_H$ (\Cref{rem:comparative statics}). Therefore, to minimise $c^*$, take: $\alpha_{2i} \to 1^{-}$, $e_S \to \infty$, and $k_H \to 1^{+}$. %Taking $\alpha_{2i} \to 1$ and $k_H \to 1$:
	\begin{align*}
		c^* \to \frac{1}{e_s - 1} \frac{1}{2} (e_S - 1) = \frac{1}{2}
	\end{align*}
	%$c_{i}^{crit} \geq \frac{1}{2}$ for all (permitted) parameter values. So for any $c^* < \frac{1}{2}$, all skilled workers want to work in high productivity firms. Therefore an equilibrium must entail $c^* \geq \frac{1}{2}$.
\end{proof}
% ------------------------------------------------------------- %



% ------------------------------------------------------------- %
% LEMMA: STATES THE EQUILIBRIUM LEVEL OF SORTING
% ------------------------------------------------------------- %
\begin{lem}\label{lem:max change in c}
	\begin{align*}
		%c^* = \frac{(\alpha_{2}^{crit})^{-1} e_S (k_H - 1) + e_S - k_H}{(e_S - 1)(k_H + 1)} \\
		\frac{d c^*}{d \alpha}\geq \frac{- e_S (k_H - 1)}{ (\alpha_{2}^{crit})^{2} (e_S -1)(k_H + 1)}
	\end{align*}
\end{lem}
% ------------------------------------------------------------- %
% PROVES THE LEMMA ABOVE
% ------------------------------------------------------------- %
\begin{proof}[\emph{\textbf{Proof of \Cref{lem:max change in c}.}}]
    Suppose $\alpha_{2i} = \alpha_2$ for all $i$ (i.e. a degenerate distribution). Then skilled workers must be indifferent between high and low productivity firms. So $\frac{1}{\alpha_{2i}} e_S (k_H - 1) = (1 + k_H) [1 + c^* (e_S - 1)] - e_S - 1$ for all $i$. Rearranging, and differentiating (and noticing that $\frac{d \alpha_{2i} }{d \alpha} = 1$) yields $\frac{d c^*}{d \alpha} = \frac{- e_S (k_H - 1)}{ (\alpha_{2}^{crit})^{2} (e_S -1)(k_H + 1)}$. \\
    
    Recall from \Cref{prop:sorting} that $c^*$ is defined by the intersection of $F(h(c))$ with the 45 degree line, and $F(h(c))$ is strictly decreasing in $c$. When $F(\cdot)$ is a degenerate distribution (i.e. it is a vertical line), then a given shift in the CDF translates into a maximal change in $c^*$. This is because $\frac{d F(h(c))}{d c} = \frac{d F(h(c))}{d h(c)} \frac{d h(c)}{d c}$, and a degenerate $F(\cdot)$ maximises $\frac{d F(h(c))}{d h(c)}$ when evaluates at $c^*$. We can also see this argument graphically.

\input{graphs/sorting_lemma_images}
%\input{tikz_pictures/sorting_lemma_graphs}

    Therefore the fall in $c^*$ is \emph{at most} that which would occur if $F(\alpha_2)$ were degenerate.
    
	%By definition $c^*$ and $\alpha_{2,eq}^{crit}$ are the values such that there is a marginal skilled worker who is indifferent between the high and low productivity firms. So when $\alpha_{2i} = \alpha_{2,eq}^{crit}$ and $c = c^*$, then \Cref{eq:firm choice ineq} is an equality. Rearranging that equation yields the first part of the Lemma.
    %The minimum value of $\frac{d c^*}{d \alpha}$ is the value what $\alpha_{2i}$ is the same for all $i$. In this case, \emph{all} skilled workers want to switch to a low productivity firm following a small change in $\alpha$ (but before $c^*$ changes to reach the new equilibrium). With heterogeneous $\alpha_{2i}$, there could be some skilled workers who do not want to switch (because they have a lower value of $\alpha_{2i}$ to begin with). Therefore, the number of skilled workers who need to switch to restore equilibrium will be \emph{weakly} lower.
\end{proof}
% ------------------------------------------------------------- %



% ------------------------------------------------------------- %
% PROVES THE OUTPUT, VARIANCE AND WELFARE RESULTS FOR THE LABOUR MARKET SORTING MODEL
% ------------------------------------------------------------- %
\begin{proof}[\emph{\textbf{Proof of Proposition \ref{prop:output,var,welfare}.}}]
Recall that $\alpha_{2i}$ is defined as a residual, while $\alpha$ and $\alpha_{1i}$ are exogenous. Therefore, $\frac{d \alpha_{2i} }{d \alpha} = 1$ and $\frac{d \alpha_{1i} }{d \alpha} = 0$ for all $i$.
\textbf{(i)} First, an increase in $\alpha$ increases $\alpha_{2i}$ for all $i$. Second, it follows from \Cref{prop:sorting} that if $\alpha_{2i}$ weakly increases for all $i$, then $c^*$ weakly decreases. Third, total output in the economy is: $y = c^* (0.5 e_S k_H + 0.5 \cdot 1) + (1 - c^*)(0.5 e_S + 0.5 k_H)$, which simplifies to: $y = 0.5 c^* (e_S k_H - e_S - k_H) + 0.5(1 + e_S + k_H)$. Clearly an increase in $c^*$ increases $y$ Therefore an increase in $\alpha$ weakly reduces total output.

\textbf{(ii)} The average wage is $\overline{w} =\gamma (0.5 \cdot c^* \cdot 1 + 0.5 \cdot (1 - c^*) \cdot k + 0.5 \cdot (1 - c^*) \cdot e + 0.5 \cdot c^* \cdot ek)$. For convenience, define $H \equiv (1 + ek - e - k)$. Using this, $\overline{w} = 0.5 \gamma [c^* H + e + k]$. Now consider the variance: %$\var(w) = E[w^2] - \overline{w}^2$
\vspace{-4mm}
\begin{align*}
	\Var(w) &= \gamma^{2} (0.5 \cdot c^* \cdot 1^{2} + 0.5 \cdot (1 - c^*) \cdot k^{2} + 0.5 \cdot (1 - c^*) \cdot e^{2} + 0.5 \cdot c^* \cdot (ek)^{2})^{2} - [0.5 \gamma (c^* H + e + k)]^{2} \\
	%\frac{2}{\gamma^{2}} \Var(w) &= c + (1 - c) \cdot k^{2} + (1 - c) \cdot e^{2} + c \cdot (ek)^{2} - 0.5 [(e+k)^{2} + c^{2} H^{2} + 2 c (e+k) H] \\
	\frac{2}{\gamma^{2}} \frac{d \Var(w)}{d c^*} &= 1 - k^{2} - e^{2} + (ek)^{2} - c^* H^{2} - (e+k) H
\end{align*}
\textbf{Aside}: it follows from straightforward manipulations that $H^{2} = (1 - k^{2} - e^{2} + (ek)^{2}) - 2 (e+k) H$.
%\begin{align*}
	%H^{2} &= (1 + ek - e - k) \cdot (1 + ek - e - k) \\
	%&= 1 + ek - e - k + ek + e^{2} k^{2} - e^{2} k - e k^{2} - e - e^{2} k + e^{2} + ek - k - e k^{2} + ek + k^{2} \\
	%&= (1 - k^{2} - e^{2} + (ek)^{2}) + (4ek - 2e - 2k - 2e^{2}k - 2ek^{2} + 2e^{2} + 2k^{2}) \\
	%&= (1 - k^{2} - e^{2} + (ek)^{2}) - 2 (e+k) (1 - e - k + ek) \\
	%&= (1 - k^{2} - e^{2} + (ek)^{2}) - 2 (e+k) H
%\end{align*}
Substituting this into the main calculation.
\begin{align*}
	\frac{2}{\gamma^{2}} \frac{d \Var(w)}{d c^*} &= (1 - k^{2} - e^{2} + (ek)^{2}) - (e+k)H - c^*([1 - k^{2} - e^{2} + (ek)^{2}] - 2(e+k)H) \\
	&= (1 - c^*) (1 - k^{2} - e^{2} + (ek)^{2}) + (2 c^* - 1)H
\end{align*}
Since $c^* \in [0.5,1]$: $(1 - c^*) \geq 0$, $(2c^* - 1) \geq 0$, and one of them must be strictly positive. Since $e > 1$, $k > 1$ (by assumption): $H > 0$. Finally, $(1 - k^{2} - e^{2} + (ek)^{2}) > 0$.\footnote{To see this, rearrange: $1 + e^{2}k^{2} > e^{2} + k^{2}$, then factorise: $(ek + 1)(ek - 1) > (e + k)(e - k)$. The first (resp. second) bracket on the LHS is larger than the first (resp. second) bracket on the RHS.}  Therefore, $\frac{d \Var(w)}{d c^*} > 0$. \\

\textbf{(iii)} There are three cases: (1) skilled worker, high productivity firm, (2) skilled worker, low productivity firm, (3) skilled worker, shifting from high productivity firm to low productivity firm (\Cref{prop:sorting} states that an increase in $\alpha$ weakly reduces $c^*$, so there will not be skilled workers shifting in the other direction). 

Utility of worker $i$ at a firm $m$ is: $u_{i}^{m} = f(Z_{im} - \alpha_{2i} \gamma \overline{w}_m )$, where $Z_{im} \equiv  \gamma e_i k_m - \alpha_{1i} \sum_{il} g_{il} w_l$. Recall that an increase in $\alpha$ weakly reduces $c^*$ (from (i)). By extension, an increase in $\alpha$ therefore weakly reduces $\overline{e}_{H}$ and weakly increases $\overline{e}_{L}$  All other terms in the utility function are constant in $\alpha$.

\noindent \textbf{Case (1).} First substitute out $\overline{e}_H = 1 + c^*(e_S - 1)$ and differentiate with respect to $\alpha$:
	\begin{align*}
		u_{S}^{H} &= f(Z_{SH} - \alpha_{2i} \gamma k_H (1 + c^* (e_S - 1)) ) \\
		\frac{d u_{S}^{H}}{d \alpha} &= f'(\cdot) \left[ - \frac{d \alpha_{2i}}{d \alpha}  \gamma k_H (1 + c^* (e_S - 1)) - \alpha_{2i} \gamma k_H (e_S - 1) \frac{d c^*}{d \alpha}  \right]  \\
		&= - f'(\cdot) \gamma k_H (e_S - 1) \left[ (e_S - 1)^{-1} + c^* + \alpha_{2i} \frac{d c^*}{d \alpha} \right]
	\end{align*}
Next, substitute in for $c^* = (e_S -1)^{-1} (k_H + 1)^{-1} \{ [(\alpha_{2,eq}^{crit})^{-1} e_S (k_H - 1)] + e_S - k_H \}$ (where \cref{eq:firm choice ineq} holds with equality) and for $\frac{d c^*}{d \alpha} = - (e_S - 1)^{-1} (k_H + 1)^{-1} [(\alpha_{2,eq}^{crit})^{-2} e_S (k_H - 1)] + \epsilon$ with $\epsilon \geq 0$ (using \Cref{lem:max change in c}):
	\begin{align*}
	%\frac{d U_{S}^{H}}{d \alpha} &= - f'(\cdot) \gamma k_H (e_S - 1) (e_S - 1)^{-1} (k_H + 1)^{-1} \left[ k_H - 1 + [(\alpha_{2,eq}^{crit})^{-1} e_S (k_H - 1)] + e_S - k_H - \alpha_{2i} [(\alpha_{2,eq}^{crit})^{-2} e_S (k_H - 1)] + \epsilon \right] \\
	\frac{d u_{S}^{H}}{d \alpha} &= - f'(\cdot) \gamma k_H (k_H + 1)^{-1} 
	        \left\{ k_H - 1 + [(\alpha_{2,eq}^{crit})^{-1} e_S (k_H - 1)] + e_S - k_H - \alpha_{2i} [(\alpha_{2,eq}^{crit})^{-2} e_S (k_H - 1)] + \epsilon  \right\} \\
	&= - f'(\cdot) \gamma k_H (k_H + 1)^{-1} 
	        \left\{ (e_S - 1) + e_S (k_H - 1) \frac{1}{\alpha_{2,eq}^{crit} } \left[ 1 - \frac{ \alpha_{2i} }{ \alpha_{2,eq}^{crit} } \right] + \epsilon \right\} \\
	\end{align*}
From \Cref{prop:network sorting}, $\alpha_{2i} \leq \alpha_{2,eq}^{crit}$ for all skilled workers who work at high productivity firms. So $1 - \frac{ \alpha_{2i} }{ \alpha_{2,eq}^{crit} } > 0$. Therefore all terms are positive (recall that $e_S > 1, k_H > 1, \gamma > 0, f'(\cdot) > 0$). So
	\begin{align*}
		\frac{d U_{S}^{H}}{d \alpha} &< 0
	\end{align*}

\textbf{Case (2)} is straightforward. An increase in $\alpha$ increases both $\alpha_{2i}$ (strictly) and $\overline{e}_{L}$ (weakly). Both of these effects reduce utility. So utility is strictly monotonically decreasing in $\alpha$. 

\textbf{Case (3).} A change from $\alpha \to \alpha'$ (with $\alpha' > \alpha$) is equivalent to a change from $\alpha_{2i} \to \alpha_{2i}^{'}$ (with $\alpha_{2i} > \alpha_{2i}^{'}$). We can break this down into two steps: (step one) $\alpha_{2i} \to \alpha_{2i}^{crit}$ and (step two) $\alpha_{2i}^{crit} \to \alpha_{2i}^{'}$. The first step is covered by case (1), the second step is covered by case (2). At $\alpha_{2i}^{crit}$ the worker is indifferent between working for the high and low productivity firms, so there is no discontinuous jump at this point. Therefore, utility is decreasing in $\alpha$. 
\end{proof}
% ------------------------------------------------------------- %


% ------------------------------------------------------------- %
% PROVES THE ENDOGENOUS NETWORK RESULT
% ------------------------------------------------------------- %
\begin{proof}[\emph{\textbf{Proof of Proposition \ref{prop:labour endo network}}}]
Denote a skilled agent working at a high productivity firm, SH. Denote an unskilled agent working at a low productivity firm UL. Denote similarly SL and UH.

Since $\alpha_{1i}$ is fixed, then adding (or strengthening) a link must be perfectly offset by weakening other links. We assume agents seek to maximise utility when choosing which link to weaken. 
Consider a UL agent, $i$. The marginal effect of strengthening a link with another UL agent, $j$, is.
\begin{align*}
    \frac{d u_i}{d g_{ij} } %= - \alpha_{1i} w_U^L f'(\cdot) + \alpha_{1i} \max \{w_l : g_{il} > 0 \} f'(\cdot) 
    = \alpha_{1i} f'(\cdot) [ \max \{w_k : g_{ik} > 0 \} - w_U^L ]
\end{align*}
because $i$ will choose to weaken a link with the agent $k$ who has the highest wage -- as this leads to the largest possible reduction in her reference point. If $i$ has any friends who are \emph{not} also of type UL, then $\max \{w_k : g_{ik} > 0 \} > w_U^L$, so she becomes strictly better off by becoming friends with another UL agent ($j$), and dropping a friendship with an agent of a different type ($k$). This logic applies to all UL type agents.

A feature of pairwise stability is that we assume a link between any pair of agents $j$ and $k$ is created it $j$ strictly prefers $g_{jk} > 0$ to $G_{jk} = 0$ and $k$ is indifferent.
%
This allows $i$ to create links with other UL-type agents until she has no non-UL-type friends left -- even if all of the other UL-type agents already have exclusively UL-type friends. This assumptions within the definition of pairwise stability prevents an agent from being ``left out''.

This logic repeats for UH, SL, and SH type agents, with the additional observation that agents with a lower income are unwilling to maintain links with others of a higher income. This means that there are no friendships across income levels, and all friendships are within a given income level.
\end{proof}
% ------------------------------------------------------------- %


==> C.further_applications.tex <==
The framework for thinking about social comparisons that we present can be applied to a wide range of other economic decisions beyond consumption and firm choice.As examples, we apply our framework to the McCall search model \citep{mccall1970search}, and to a static CAPM. These are very simple models that look at wage determination and asset allocations, respectively.\footnote{Education decisions are another scenario where social comparisons would be important. We do not present such an application as, in practice, it would overlap with the extensive literature on peer effects. Closest to our framework is \cite{calvo2009peer}, but the literature is extensive (see \cite{durlauf2004neighborhood} and \cite{epple2011peer} for reviews.}

\subsection{Portfolio allocation}\label{subsec:financial markets}
\noindent \textbf{Model.} There are two assets in the economy: a risk-free asset (`debt'), with a gross return $r_{f} = 1$, and a risky asset (`equity'), with a random gross return $r_{e}$. $r_e$ follows a cumulative distribution function $G(r_{e})$, with $G(0) = 0$ and $\int r_e d G(r_e) > 1$. The ex-post equity premium is $r_{p} \equiv r_{e} - r_{f}$. Returns are common to all agents. All agents $i$ have (the same) initial wealth $w$. After returns are realised, all wealth is consumed. Agents have reference dependent preferences over final consumption, as in Section \ref{sec:results}. They must allocate a fraction $\lambda_{i}$ of wealth to equity, and the rest to debt. The agent's problem is:

\begin{align*}
	u_{i}(x_{i} , x_{-i}) &= \mathbb{E}[f(x_{i} - \alpha_i \sum_{j} g_{ij} x_{j} )]
	\qquad \text{ subject to } \qquad
	x_{i} = w ( r_{f} + \lambda_{i} r_{p} ) \ \forall i
	%u_{i}(c_{i} , c_{-i}) &= \mathbb{E} \left[ f( w (1 - \alpha_i) + w (r_{e} - 1) ( \lambda_{i} - \sum_{j} G_{ij} \lambda_{j} ) ) \right] \\
\end{align*}

Let $\rho = \frac{- f''(z)}{f'(z)}$ be the \emph{coefficient of relative absolute aversion} (defined in the usual way, see for example \citet[Chapter 6.C]{mas1995microeconomic}). We can now show how agents' social comparisons affect their portfolio allocation decisions.

%If there is an interior solution, this yields the First Order Condition: $\mathbb{E}[ f'(\cdot) (r_{e} - 1) w ]  = 0$.\footnote{This is straightforward, but for completeness, we show this in Appendix \ref{proofs: footnotes}. \label{footnote CAPM FOC}}
%\begin{align*}
%	\mathbb{E}[ f'( %w (1 - \alpha_i) + w (r_{e} - 1) ( \lambda_{i} - \sum_{j} G_{ij} \lambda_{j} )) \cdot
%	\cdot) (r_{e} - 1) w ]  = 0
%\end{align*}

\begin{prop}\label{prop:portfolio allocation}
    Suppose agents allocate wealth to both bonds and equities, and that the utility function $f(\cdot)$ exhibits decreasing absolute risk aversion. Then an increase in the strength of social comparisons, $\alpha_i$, strictly reduces the amount of wealth agent $i$ allocates to equities, and weakly reduces the amount all other agents allocate to equities.
\end{prop}

When an agent make stronger social comparisons with her neighbours, then she feels as if she is poorer. This is because her consumption is (all else equal) closer to her reference point. She then behaves as if she has less wealth. With decreasing relative risk aversion, effective lower wealth makes an agent more risk averse, and so she allocates less wealth to risk assets (equities).\footnote{With few constraints on the functional form we cannot find a closed-form solution for the optimal allocation. In the online appendix, we consider the case of quadratic utility. This permits a closed-form solution, and exhibits \emph{increasing} relative risk aversion -- so it shows an inverted qualitative result.}

While this is only a partial equilibrium model, as the prices of the two assets are assumed to be exogenous, the effect on asset prices is straightforward. For a \emph{given} set of prices, stronger social comparisons reduce allocations to equities and increase allocations to bonds. This would then reduce equity prices and increase bond price, in turn  inducing agents to allocate more wealth to equities and less to bonds. This would re-establish market clearing for the assets. Therefore, with decreasing relative risk aversion, stronger social comparisons will raise risk premia. 

This result is closely related to \cite{gali1994keeping}, who also examines social dimensions to investment decisions. \cite{gali1994keeping} studies a setting where agents have preferences over their own consumption and average consumption in the economy. It also complements models of external habit-formation in financial markets (for example \cite{abel1990asset, grishchenko2010internal, campbell1999force}). Instead of having utility depend on other agents' \emph{past} consumption, our result looks at the case where utility depends on other agents' \emph{current} consumption.

Finally, we present an analogy to \Cref{prop:portfolio allocation} when agents have quadratic utility. This allows for a closed form solution. Note, however, that a quadratic utility function exhibits \emph{increasing} absolute risk aversion, and so the result is in the other direction to \Cref{prop:portfolio allocation}.
\begin{prop}\label{prop:portfolio extension}
    Let $f(z_i) \approx a_0 + a_1 z_i + a_2 z_i^2$, with $a_1 > 0$, $a_2 < 0$, $z_i = x_i - \alpha_i \sum_j g_{ij} x_j$ and $x_i = w (1 + \lambda_i r_p)$ for all $i$. Then:
\begin{align*}
\lambda^{*}_{i} &= \left[ \left( \frac{-a_{1}}{2 a_{2} w} + (\overline{\alpha} - 1) r_{f} \right) \frac{ \mathbb{E}[r_{p}] }{ \mathbb{E}[r_{p}^{2}]  } \right] C^{b}_{i} + \left[ r_{f} \frac{\mathbb{E}[r_{p}] }{\mathbb{E}[r_{p}^{2}] } \right] \Cov( B_{ij} , \alpha_{j} ) 
\end{align*}
\end{prop}


% ------------------------------------------------------------------------- %
\subsection{Wages: McCall Model}\label{subsec:labour markets}
We present the standard McCall search model \citep{mccall1970search} with one difference. Instead of having linear preferences over her wage, an agent has non-linear preferences over her wage relative to some weighted average of her friends' wages (her reference point). \\

\noindent \textbf{Model.} A risk neutral agent searches for a job. In a period where she searches, she receives one job offer with a wage $w \stackrel{i.i.d}{\sim} G(\hat{w})$, with $G(0) = 0$ and $G(Z) = 1$ (where $G(\hat{w})$ is a continuous probability density function) for some $Z < \infty$. $G(w)$ is known ex ante. After receiving the offer, the worker observes $x$ and then chooses whether to \textit{accept} the offer, or \textit{reject} it and search again. Once accepted, the job lasts forever. The agent has preferences;
\begin{align*}
u_{i}(w_{i} , R_{i}) = \sum_{t=0}^{\infty} \beta^{t} \cdot f \left( w_{it} - R_{i}  \right)
\end{align*}
Where $R_{i}$ is the reference point, $f(\cdot)$ is a strictly concave function, $\beta \in (0,1)$ is her discount factor. \\

\noindent \textbf{Exogenous reference point.} First, we consider an agent with an exogenous reference point. We can think of this as a setting where agents searching for jobs \emph{sequentially}, so agent $i$'s reference point is determined only from neighbours who already have a job. The key point here is that an agent's reference point is \emph{fixed} when she searches for a job.\footnote{Intuitively, this corresponds to a cohort of new job seekers forming their reference point from an already-employed cohort. In practice, this might correspond to people forming a reference point from their parents or recent graduates of their school/university.} This suppresses general equilibrium effects -- i.e. the feedback loop, where $i$'s decision affects $j$'s decision, which in turn affects $i$'s. This significantly aids tractability, and allows for general analytic solutions. As there is only one agent (at a time) here, we will suppress the $i$ subscripts for convenience. %In the standard McCall search model, there is no closed-form solution the reservation wage, so it is not surprising that closed-form solutions are also unavailable here.\footnote{See, for example, \citet[Section 6.3, pages 163-7]{ljungqvist2012recursive}.}

\begin{prop}\label{prop:res wage exogeneous}
An agent's reservation wage, $\overline{w}$, solves the equation
\begin{align}\label{eq:mccall eq 1}
f \left(\overline{w} - R \right) =
 	 \frac{ \beta }{ 1 - \beta } \int_{\overline{w}}^{Z}   [ f \left( w' - R \right) - f \left( \overline{w} - R \right) ] d G(w')
\end{align}
and is strictly monotonically increasing in their reference point $R$, but less than proportionately
\begin{align*}
0 < \frac{d \overline{w}}{ d R} < 1
\end{align*}
\end{prop}

This result shows that the standard equation defining the reservation wage in the McCall model extends straightforwardly to the setting with social comparisons.\footnote{We have omitted the unemployment benefits as they are not important for this model. Adding them in complicates the algebra, but does not yield any insight.} There is now the addition of the reference point. As an agent's reference point increases, her reservation wage increases. A higher reference point raises the costliness of searching for another period, and reduces the benefits of accepting a job at a given wage. Overall, the second effect dominates -- it is worse to be locked into a wage that is `too low' than to wait another period.

A higher reference point causes agents to search for longer to find a job, and to earn higher wages (on average). Recall that we interpret the reference point that as a weighted mean of neighbours' wages, scaled by some reference strength. This result suggests that agents who have higher earning neighbours and/or make stronger social comparisons spend more time searching for a job, and will be rewarded for this with a higher wage. \\

\noindent \textbf{Endogenous reference point.} We might also be interested in a world where agents to choose their reservation wages \emph{simultaneously}. This re-introduces the general equilibrium effects that we suppressed in order to state \Cref{prop:res wage exogeneous}. However, this significantly complicates the model, and prevents clean comparative statics. Nevertheless, we can say that equilibrium reservation wages exist and are unique when the strength of social comparisons is not too strong.

\begin{prop}\label{prop:res wage endogenous}
Suppose $\alpha_{i} < 1$ for all agents. Then there is a unique equilibrium set of reservation wages, $y^{*}$.
\end{prop}

The logic is the same as for \Cref{prop:equilibrium} -- the spillover effects must eventually `die out'. Otherwise agents would be forced into a competitive spiral where they hold out forever for the absolute highest wage available.\footnote{Which is a probability zero event, as the density function of job offers is continuous.} Further analytic results are unavailable, but simulations in the Online Appendix show that an agent's optimal reservation wage is very closely linked to her Bonacich centrality. Linear combinations of agents' Bonacich centralities and their reference strengths together explain almost all of the variation in equilibrium reservation wages. 


\subsection{Simulations}\label{sec:simulations}
We were unable to show a closed-form solution for the optimal reservation wage with an endogenous reference point. Given what we have learned so far about the effects of social comparisons, we expect that the strength of agents' social comparisons and their Bonacich centralities will play a crucial role in determining the reservation wage. To test this conjecture, we solve the model using computational methods. First, we use simulation methods to generate a sample of networks. Second, we use standard computational methods to solve the model for each network in the sample. Finally, we use regression analysis to look for a relationship between the reservation wage and Bonacich centrality and reference strength.

For simulating networks, we use Erd{\"o}s-R{\'e}nyi random graphs \citep{erdos1959random}, a seminal model of random graphs. In this model, there are $n$ agents, and each possible link between two agents present uniformly at random with probability $p$ (and not present with probability $1- p$). It generates an \emph{unweighted} graph. In our simulations, we have $n=50$ agents and $p = 0.2$.

After randomly generating the links, we uniformly scale down their weights such that $g$ is a Markov chain (so if agent $i$ has $d_i^{out}$ outward links, then each link has a weight $\frac{1}{d_i^{out}}$). This makes the network structure weighted. Note that this scaling down is a small variant on the seminal model. For a given agent, all of their outward links have the same weight, but the link weights will differ across agents. This is because they have different numbers of neighbours, due to the random generation of the links. %This is an extremely simplistic model, but nevertheless has all of the key features we need.

We then randomly generate a \emph{reference strength}, $\alpha_i$. Here, an agent's reference strength is drawn randomly from the uniform distribution on $[0.4, 0.8]$. We also need some other parameters for the reservation wage part. We fix the maximum wage offer at $Z = 100$, the discount factor at $\beta = 0.98$, and the functional form of $f(x) = x^{0.25}$. Note that there is no cost parameter, $c$ in this model.

Taking one simulated network, we calculate the optimal reservation wages using the following algorithm.
\begin{enumerate}
    \item Take an initial guess at the reservation wage for each agent.
    \item Given all agents' reservation wages, calculate their reference points, by multiplying the network $G$ by the vector of reservation wages.
    \item Take one agent, and treat her reference point as fixed. Calculate her optimal reservation wage.\footnote{This is not computationally straightforward. For a given value of $y$, calculate the Left-Hand Side and Right-Hand Side of \Cref{eq:mccall eq 1} separately, using numerical integration -- this yields the difference between the Left-Hand Side and Right-Hand Side. Then use the Newton-Raphson method to find the value of $y$ that solves the equation. Store this as the ``updated'' reservation wage.}
    \item Repeat step 3 for each agent in the network. 
    \item Repeat steps 2-4 until the process converges.
\end{enumerate}
This algorithm must be applied to each simulated network in in the sample. It is computationally intensive, so we have restricted the network to 50 agents.

Simulations followed by computational methods yield an optimal reservation wage, Bonacich centrality, and reference strength for each agent. With 1,000 distinct networks, and 50 agents per network, we have a sample of 50,000 observations. We perform Ordinary Least Squares regression to look for a simple linear relationship between optimal reservation wages, and Bonacich centrality and reference strength. The aim is to see whether these two factors can explain most of the variation in reservation wages. Therefore, we are interested in the R-squared of the regressions. This is somewhat atypical. However, we are using the outputs of a \emph{theoretical model} to look for a relationship between variables within that model. We are \emph{not} looking for causal relationships within actual data. \\ %Given this, it is most interesting to look at a regression without a constant term -- as this directly considers whether the optimal reservation wage appears to be a function of Bonacich centrality and reference strength alone. \\

\noindent \textbf{Results.} Our conjecture is that an agent's optimal reservation wage is a function of her Bonacich centrality and her reference strength. Before turning to regression analysis, it is immediately obvious from simple scatter plots of reservation wages against Bonacich centralities and against reference strengths (Figures \ref{fig: res wage:a} and \ref{fig: res wage:b} respectively) that there is a very close relationship between the optimal reservation wage and both the reference strength and Bonacich centrality. 

\vspace{10mm}

\begin{figure}[H]
    %\centering
    \caption{Optimal reservation wage and network centrality measures}\label{fig: res wage}
    \vspace{2mm}
    \begin{subfigure}[t]{0.5\textwidth}
    %\hspace{-20mm}
    \includegraphics[width=8cm]{res_wage_vs_bonacich}
    \caption{Bonacich centrality}\label{fig: res wage:a}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.5\textwidth}
    \centering
    \includegraphics[width=8cm]{res_wage_vs_alpha}
    \caption{Reference strength}\label{fig: res wage:b}
    \end{subfigure}
\end{figure}

Regression analysis confirms this. The two variables, even when only included linearly, together explain over 99\% of the variation in the optimal reservation wage. Formally, in an OLS regression of reservation wage on Bonacich centrality and reference strength without a constant, we get an $R^{2}$ value of $0.995$ (with a constant, it rises to $0.998$).

\begin{table}[H]
\centering
\caption{OLS Regression Results: No constant}
	\begin{tabular}{lcccccc}
\toprule
                     & \textbf{coef} & \textbf{std err} & \textbf{t} & \textbf{P$> |$t$|$} & \textbf{[0.025} & \textbf{0.975]}  \\
\midrule
\textbf{r\_bonacich} &      52.9210  &        0.122     &   433.400  &         0.000        &       52.682    &       53.160     \\
\textbf{alpha}       &     -95.7810  &        0.506     &  -189.201  &         0.000        &      -96.773    &      -94.789     \\
\bottomrule
	\end{tabular}
\end{table}

\noindent \textbf{R-squared (uncentered):} 0.995 , \textbf{Adj.R-squared (uncentered):} 0.995 , \textbf{F-statistic:} 4.730e+06 \\


\vspace{5mm}
\begin{table}[H]
\centering
\caption{OLS Regression Results: With constant}
	\begin{tabular}{lcccccc}
\toprule
                     & \textbf{coef} & \textbf{std err} & \textbf{t} & \textbf{P$> |$t$|$} & \textbf{[0.025} & \textbf{0.975]}  \\
\midrule
\textbf{const}       &      62.0461  &        0.005     &  1.16e+04  &         0.000        &       62.036    &       62.057     \\
\textbf{r\_bonacich} &       1.5872  &        0.005     &   317.294  &         0.000        &        1.577    &        1.597     \\
\textbf{alpha}       &      16.5772  &        0.014     &  1208.692  &         0.000        &       16.550    &       16.604     \\
\bottomrule
	\end{tabular}
\end{table}

\noindent \textbf{R-squared (uncentered):} 0.998 , \textbf{Adj.R-squared (uncentered):} 0.998 , \textbf{F-statistic:} 1.282e+07  \\




\subsection{Proofs}
% ------------------------------------------------------------- %
% PROVES THAT WITH DECREASING RELATIVE RISK AVERSION, HIGHER ALPHA REDUCES ALLOCATION TO RISKY ASSETS
% ------------------------------------------------------------- %
\begin{proof}[\emph{\textbf{Proof of Proposition \ref{prop:portfolio allocation}}}]
Substitute the constraint into the utility function, and W.L.O.G let $r_f = 1$. 
\begin{align*}
    u_{i}(x_{i} , x_{-i}) &= \mathbb{E}[f(w (1 - \alpha_i) + w r_p (\lambda_i - \alpha_i \sum_{j} g_{ij} \lambda_{j}))]
\end{align*}
Notice that for an interior equilibrium to exist, there must be some positive probability that $r_p < 0$ (otherwise the risky asset would always have a higher return than the risk-free asset). Supposing that an interior equilibrium exists, then at the equilibrium:
\begin{align*}
    \frac{d u_i}{d \lambda_i} &= \mathbb{E}[ w r_p f'(w (1 - \alpha_i) + w r_p (\lambda_i - \alpha_i \sum_{j} g_{ij} \lambda_{j}))] = 0 %\\
    %&= \mathbb{E}[ w r_p f'(z) | r_p > 0] + \mathbb{E}[ w r_p f'(z) | r_p < 0]
\end{align*}
where $z_i \equiv w (1 - \alpha_i) + w r_p (\lambda_i - \alpha_i \sum_{j} g_{ij} \lambda_{j})$ is \emph{effective wealth}. A well-known result is that when an agent has a utility function with decreasing absolute risk aversion, then she allocates more of her portfolio to the risky asset as her wealth rises (see for example, \cite[Exercise 6.C.8]{mas1995microeconomic}). 

Note that $f'(z)$ is strictly monotonically decreasing in $z$.

Now suppose that $\alpha_i$ increases (for some $i$). Then $z$ decreases, since:
\begin{align*}
    \frac{d z_i}{d \alpha_i} = - w (1 + r_p \sum_{j} g_{ij} \lambda_j
\end{align*}
which is negative because $\lambda_j \leq 1$ for all $j$ (because an agent cannot invest more than all of her wealth in the risky asset), $\sum_j g_{ij} = 1$ by construction, and $r_p > -1$ in all instances by assumption. Therefore \emph{effective wealth} decreases, which makes $i$ agent more risk averse (in absolute terms), so she allocates less wealth to risky assets.

We now need to consider all other agents. Consider a typical agent $k \neq i$. $\lambda_i$ falls (in response to the increase in $\alpha_i$). 
\begin{align*}
    \frac{d \mathbb{E}[w r_p f'(z_k)}{d \lambda_j} &= \mathbb{E}[- \alpha_k g_{kj} w^2 r_p^2 f''(z_k)] > 0
\end{align*}
since $f''(z) < 0$ (by concavity of $f(z)$). So reduction in $\lambda_j$ requires an adjustment in $\lambda_k$ to return to the equilibrium condition. In particular, it requires a reduction in $\lambda_k$. This is because:
\begin{align*}
    \frac{d \mathbb{E}[w r_p f'(z_k)}{d \lambda_k} &= \mathbb{E}[w^2 r_p^2 f''(z_k)] < 0
\end{align*}
Therefore investment in the risky asset is complementary across agents. An increase in $\alpha_i$ causes agent $i$ to invest less in the risky asset. In turn, all other agents invest less in the risky asset.
\end{proof}



\begin{proof}[\emph{\textbf{Proof of Proposition \ref{prop:portfolio extension}}}]
First, note that expectations and differentials are both linear operators, so we can interchange order. Next, use the quadratic utility representation, and then notice that the expectation operator only acts on the $r_p$ terms (allowing us to bring the expectation operator through).
\begin{align*}
\frac{\delta u_{i} }{\delta \lambda_{i}} 
    &= \frac{\delta}{\delta \lambda_{i}} \mathbb{E}[f(z_i)]
    = \mathbb{E} \left[ \frac{\delta  f(z_i)}{\delta \lambda_{i}} \right] 
    = \mathbb{E} \left[ \frac{\delta f(z_i) }{\delta z_i } \frac{\delta z_i }{\delta \lambda_{i} }  \right] \\
\frac{\delta u_{i} }{\delta \lambda_{i}} &= \mathbb{E}[(a_{1} + 2 a_{2} z_i) \cdot w r_{p}] \\
&= \mathbb{E}[a_{1} w r_{p} + 2 a_{2} w^{2} r_{p} \ r_{f} (1 - \sum_{j} G_{ij}) + 2 a_{2} w^{2} r_{p}^{2} ( \lambda_{i} - \sum_{j} G_{ij} \lambda_{j} )] \\
&= a_{1} w \mathbb{E}[r_{p}] + 2 a_{2} w^{2} \mathbb{E}[r_{p}] \ r_{f} (1 - \sum_{j} G_{ij})
	+ 2 a_{2} w^{2} \mathbb{E}[r_{p}^{2}] ( \lambda_{i} - \sum_{j} G_{ij} \lambda_{j} )
\end{align*}
Set equal to zero, getting the First Order Condition. Then rearrange and recall that $(1-\sum_{j} G_{ij}) = \alpha_{i}$.
\begin{align*}
0 &= a_{1} w \mathbb{E}[r_{p}] + 2 a_{2} w^{2} \mathbb{E}[r_{p}] \ r_{f} (1 - \sum_{j} G_{ij})
	+ 2 a_{2} w^{2} \mathbb{E}[r_{p}^{2}] ( \lambda_{i}^{*} - \sum_{j} G_{ij} \lambda_{j}^{*} ) \\
%( \lambda_{i}^{*} - \sum_{j} G_{ij} \lambda_{j}^{*} ) &=
%	- \frac{ a_{1} w \mathbb{E}[r_{p}] }{2 a_{2} w^{2} \mathbb{E}[r_{p}^{2}]  }
%	- \frac{2 a_{2} w^{2} \mathbb{E}[r_{p}] \ r_{f} }{ 2 a_{2} w^{2} \mathbb{E}[r_{p}^{2}] }
%			\cdot (1-\sum_{j} G_{ij}) \\
%( \lambda_{i}^{*} - \sum_{j} G_{ij} \lambda_{j}^{*} ) &=
%	- \frac{ a_{1} \mathbb{E}[r_{p}] }{2 a_{2} w \mathbb{E}[r_{p}^{2}]  }
%	- \frac{ r_{f} \mathbb{E}[r_{p}] }{\mathbb{E}[r_{p}^{2}] }
%			\cdot ( 1 - \alpha_{i}) \\
( \lambda_{i}^{*} - \sum_{j} G_{ij} \lambda_{j}^{*} ) &=
	\left( \frac{-a_{1}}{2 a_{2} w} - r_{f} \right) \frac{ \mathbb{E}[r_{p}] }{ \mathbb{E}[r_{p}^{2}]  }
	+ r_{f} \alpha_{i} \frac{\mathbb{E}[r_{p}] }{\mathbb{E}[r_{p}^{2}] }
\end{align*}

\noindent In matrix form
\begin{align*}
( \lambda^{*} - G \lambda^{*} ) &=
	\left[ \left( \frac{-a_{1}}{2 a_{2} w} - r_{f} \right) \frac{ \mathbb{E}[r_{p}] }{ \mathbb{E}[r_{p}^{2}]  } \right] \cdot \mathbf{1}
	+ \left[ r_{f} \frac{\mathbb{E}[r_{p}] }{\mathbb{E}[r_{p}^{2}] } \right] \cdot \alpha \\
\lambda^{*} &= \left[ \left( \frac{-a_{1}}{2 a_{2} w} - r_{f} \right) \frac{ \mathbb{E}[r_{p}] }{ \mathbb{E}[r_{p}^{2}]  } \right] (I - G)^{-1} \cdot \mathbf{1}
		+ \left[ r_{f} \frac{\mathbb{E}[r_{p}] }{\mathbb{E}[r_{p}^{2}] } \right] (I - G)^{-1} \cdot \alpha
\end{align*}

\noindent For an individual agent
\begin{align*}
\lambda^{*}_{i} &= \left[ \left( \frac{-a_{1}}{2 a_{2} w} - r_{f} \right) \frac{ \mathbb{E}[r_{p}] }{ \mathbb{E}[r_{p}^{2}]  } \right] \sum_{j} B_{ij}
+ \left[ r_{f} \frac{\mathbb{E}[r_{p}] }{\mathbb{E}[r_{p}^{2}] } \right]  \sum_{j} B_{ij} \alpha_{j} \\
%\lambda^{*}_{i} &= \left[ \left( \frac{-a_{1}}{2 a_{2} w} - r_{f} \right) \frac{ \mathbb{E}[r_{p}] }{ \mathbb{E}[r_{p}^{2}]  } \right] \sum_{j} B_{ij}
%+ \left[ r_{f} \frac{\mathbb{E}[r_{p}] }{\mathbb{E}[r_{p}^{2}] } \right] \left[ \frac{1}{n} \sum_{j} B_{ij} \sum_{j} \alpha_{j} + \Cov( B_{ij} , \alpha_{j} ) \right] \\
\lambda^{*}_{i} &= \left[ \left( \frac{-a_{1}}{2 a_{2} w} - (1 - \overline{\alpha}) r_{f} \right) \frac{ \mathbb{E}[r_{p}] }{ \mathbb{E}[r_{p}^{2}]  } \right] C^{b}_{i}
+ \left[ r_{f} \frac{\mathbb{E}[r_{p}] }{\mathbb{E}[r_{p}^{2}] } \right] \Cov( B_{ij} , \alpha_{j} )
\end{align*}
\end{proof}


% ------------------------------------------------------------- %
% PROOF THAT MCCALL MODEL STILL WORKS (DE FACTO) UNCHANGED WHEN THE REFERENCE POINT IS EXOGENOUS
% ------------------------------------------------------------- %
\begin{proof}[\emph{\textbf{Proof of Proposition \ref{prop:res wage exogeneous}.}}]
The first part of the proposition follows from the standard derivation of the basic McCall search model (without unemployment benefits). See for example \cite[Chapter 6.3]{ljungqvist2012recursive}. The only change is that it uses $f(w - R)$ in place of $w$, and $f(\overline{w} - R)$ in place of $\overline{w}$. Therefore we omit the working here (it is provided in the Online Appendix for completeness).

Next, we prove that the partial derivative of $\overline{w}$ with respect to $R$ is strictly between $0$ and $1$. Start with the reservation wage equation. Then separate out the two terms in the RHS integral, resolve the second integral created by the separation, notice that $G(Z) = 1$, and $G'(x) \equiv g(x)$, and rearrange terms.
%\begin{align*}
%f(\overline{w} - R) = \frac{\beta}{1 - \beta} \int_{\overline{w}}^{Z} [ f( w' - R) - f( \overline{w} - R) ] d G(w')
%\intertext{Rearranging }
%\frac{1 - \beta}{\beta} \cdot f(\overline{w} - R) = \int_{\overline{w}}^{Z} f(w' - R) d G(w') - f(\overline{w} - R) \int_{\overline{w}}^{Z} d G(w')
%\intertext{Resolving the final integral, and noticing that $G(Z) = 1$ }
%\frac{1 - \beta}{\beta} \cdot f(\overline{w} - R) = \int_{\overline{w}}^{Z} f(w' - R) d G(x') - f(\overline{w} - R) (1 - G(\overline{w})) \\
%\left( \frac{1}{\beta} - G(\overline{w}) \right) \cdot f(\overline{w} - R) = \int_{\overline{w}}^{Z} f(w' - R) d G(w')
%\end{align*}
%\noindent Let $g(w) \equiv G'(w)$, then;
\begin{align}\label{mccall eq 2}
\left( \frac{1}{\beta} - G(\overline{w}) \right) \cdot f(\overline{w} - R) = \int_{\overline{w}}^{Z} f(w' - R) g(w') d w'
\end{align}

W.L.O.G. let $M(R,\overline{w},Z) \equiv \int_{\overline{w}}^{Z} f(w' - R) g(w') d w'$, and let $\frac{\delta S(w',R)}{\delta w'} \equiv f(w' - R) g(w')$. So $S(Z,R) - S(\overline{w},R) = M(R,\overline{w},Z)$. Therefore $M'_{\overline{w}}(R,\overline{w},Z) = - S'(\overline{w},R) = - f(\overline{w} - R) g(\overline{w})$. Now, totally differentiate equation \ref{mccall eq 2}, and substitute in $M'_{\overline{w}}(R,\overline{w},Z) = - f(\overline{w} - R) g(\overline{w})$.
\begin{align*}
    \frac{\delta LHS}{\delta \overline{w}} d\overline{w} +  \frac{\delta LHS}{\delta R} dR 
    &= \frac{\delta RHS}{\delta \overline{w}} d\overline{w} +  \frac{\delta RHS}{\delta R} dR \\
    \left[ \left( \frac{1}{\beta} - G(\overline{w}) \right) \cdot f'(\overline{w} - R) - g(\overline{w}) f(\overline{w} - R) \right] d\overline{w} \quad& \\
- \left( \frac{1}{\beta} - G(\overline{w}) \right) \cdot f'(\overline{w} - R) dR &=
- f(\overline{w} - R) g(\overline{w}) d\overline{w} + M^{'}_{R}(R,\overline{w},Z) dR
\end{align*}
Simplifying and rearranging yields
\begin{align}\label{mccall eq 3}
\frac{d\overline{w}}{dR} = 1 + \frac{ M^{'}_{R}(R,\overline{w},Z) }{ \left( \frac{1}{\beta} - G(\overline{w}) \right) \cdot f'(\overline{w} - R) }
\end{align}

Now we show bounds on $M^{'}_{R}(R,\overline{w},Z)$. \textit{Lower bound.} Note that we can interchange order of differentiation and integration, so $M^{'}_{R}(R,\overline{w},Z) = \int_{\overline{w}}^{Z} - f'(w' - R) g(w') dw'$. Recall that $f(\cdot)$ is strictly concave, so $f'(\cdot)$ is strictly decreasing. Therefore $f'(\overline{w} - R) > f'(w' - R)$ for all $w' > \overline{w}$. We are integrating between $\overline{w}$ and $Z$ (which is larger than $\overline{w}$ by construction). Therefore:
\begin{align}
    M^{'}_{R}(R,\overline{w},Z) > - f'(\overline{w} - R) (1 - G(\overline{w}))
\end{align}
\textit{Upper bound.} By an identical argument $f'(Z - R) > f'(w' - R)$ for all $w' < Z$. Therefore:
\begin{align}
    M^{'}_{R}(R,\overline{w},Z) < - f'(Z - R) (1 - G(\overline{w}))
\end{align}
Using the lower bound and rearranging terms:
\begin{align*}
    %\frac{d\overline{w}}{dR} > 1 + \frac{ - f'(\overline{w} - R) (1 - G(\overline{w})) }{ \left( \frac{1}{\beta} - G(\overline{w}) \right) \cdot f'(\overline{w} - R) } \\
    \frac{d\overline{w}}{dR} &> 1  - \beta \frac{1 - G(\overline{w}) }{1 - \beta G(\overline{w})} \\
    \frac{d\overline{w}}{dR} &> \frac{1 - \beta}{1 - \beta G(\overline{w}) } > 0
\end{align*}
Since $\beta < 1$ and $G(\overline{w}) < 1$. Using the upper bound:
\begin{align*}
    \frac{d\overline{w}}{dR} &< 1 + \frac{ - f'(Z - R) (1 - G(\overline{w}) ) }{ \left( \frac{1}{\beta} - G(\overline{w}) \right) \cdot f'(\overline{w} - R) } \\
    \frac{d\overline{w}}{dR} &< 1 + \underbrace{\left( \frac{1 - \beta}{ 1 - \beta G(\overline{w})} - 1 \right)}_{\in (-1,0)}  \cdot \underbrace{\frac{f'(Z - R)}{f'(\overline{w} - R)} }_{\in (0,1)} < 1
\end{align*}
Since $\beta < 1$ and $G(\overline{w}) < 1$, and since $f'(Z - R) < f'(\overline{w} - R)$. This proves both bounds as required.
\end{proof}
% ------------------------------------------------------------- %



% ------------------------------------------------------------- %
% STATES BROUWER'S FIXED POINT THEOREM
% ------------------------------------------------------------- %
\begin{thm}[Brouwer's Fixed Point Theorem]
Let $S$ be a non-empty, convex and compact subset of $\mathbb{R}^{n}$. If $f:S \to S$ is continuous, then $f$ has a fixed point.
\end{thm}
% ------------------------------------------------------------- %


% COMMENT ON NOTATION FOR THE ENDOGENOUS REFERENCE POINT MCCALL MODEL PROOF
Before proving \Cref{prop:res wage endogenous}, it is helpful to clarify some notation. For the purposes of the proof to \Cref{prop:res wage endogenous} Variables without a subscript (e.g. $\overline{w}, R, x$) are $n \times 1$ column vectors. Variables with a subscript (e.g $\overline{w}_{i}, D_{k}$) are scalars, and are typically elements from a corresponding vector. $f(\cdot)$ and $H(\cdot)$ are functions. In a small abuse of notation, when the argument is a scalar, or collection of scalars, the output is a scalar. When the argument is a vector, the output is a vector.
% ------------------------------------------------------------- %
% PROVES THAT OPTIMAL RESERVATION WAGES EXIST WHEN REFERENCE POINTS ARE ENDOGENOUS
% ------------------------------------------------------------- %
\begin{proof}[\emph{\textbf{Proof of Proposition \ref{prop:res wage endogenous}.}}]
There is a different reservation wage equation for each agent, and the reference point is a function of other agents' reservation wages. The analogous equation to \Cref{prop:res wage exogeneous} is:
\begin{align}\label{mccall eq 4}
f \left(\overline{w}_{i} - \alpha_{i} \sum_{j} G_{ij} \overline{w}_{j} \right) =
 	 \frac{ \beta }{ 1 - \beta } \int_{\overline{w}_{i}}^{Z}   \left[ f \left( w' - \alpha_{i} \sum_{j} G_{ij} \overline{w}_{j} \right) - f \left( \overline{w}_{i} - \alpha_{i} \sum_{j} G_{ij} \overline{w}_{j} \right) \right] d G(w')
\end{align}
By the Implicit Function Theorem, we can write $\overline{w}_{i} = H( \overline{w}_{-i} )$. Then considering this system of equations as a single equation with a vector input and vector output, we can write $H(\overline{w}) = \overline{w}$. We now show that this equation has a unique fixed point.

\textbf{Existence.} Notice that $H: W \to W$, where $W = [0 , Z]^{n}$. Therefore, $W$ is a non-empty, convex and compact subset of $\mathbb{R}^{n}$. Recall $f(\cdot)$ is everywhere continuous by assumption. Integration, addition and subtraction (as performed in equation \ref{mccall eq 4}) preserves continuity, so $H:WY \to W$ is also continuous. Therefore, $H: W \to W$ satisfies the requirements of Brouwer's Fixed Point Theorem, and so has at least one fixed point.

\textbf{Uniqueness.} We know from above that at least one fixed point exists. Denote the smallest fixed point $\overline{w}^{*}$. So $H(y^{*}) = y^{*}$. Now suppose that there exists another fixed point, $(\overline{w}^{*} + D)$ (with $i^{th}$ element $(\overline{w}^{*} + D)_{i} = \overline{w}^{*}_{i} + D_{i}$). W.L.O.G. suppose that the $k^{th}$ element exhibits the largest increase vis-a-vis $\overline{w}^{*}$. We now focus on the $k^{th}$ equation. By the Mean Value Theorem
${H(\overline{w}^{*}_{-k} + D_{-k}) = H(\overline{w}^{*}_{-k}) + \nabla H(\overline{w}^{*}_{-k} + c D_{-k}) \cdot D_{-k} \ \text{ for some } \ c \in [0,1]}$. By the rules of total differentiation:
\begin{align*}
\nabla H(\overline{w}^{*}_{-k} + cD_{-k}) \cdot D_{-k} = \sum_{i \neq k} \frac{\delta H(\overline{w}^{*}_{-k} + c D_{-k})}{\delta \overline{w}_{i}} D_{i}  \leq D_{k} \sum_{i \neq k} \frac{\delta H(\overline{w}^{*}_{-k} + cD_{-k})}{\delta \overline{w}_{i}}
\end{align*}
Since $D_{i} \leq D_{k}$ for all $i \neq k$ by construction. From Proposition \ref{prop:res wage endogenous}: $\frac{\delta \overline{w}_{k}}{\delta R_{k}} < 1$. By the chain rule (and the definition of $R_{i}$), $\frac{\delta \overline{w}_{k}}{\delta \overline{w}_{i}} = \frac{\delta \overline{w}_{k}}{\delta R_{k}} \frac{\delta R_{k}}{\delta \overline{w}_{i}} < G_{ki}$ for all $i, k$. Note that $\overline{w}_{k} \equiv H(\overline{w}_{-k})$. So $\frac{\delta H(\overline{w}_{-k})}{\overline{w}_{i}} \equiv \frac{\delta \overline{w}_{k}}{\delta \overline{w}_{i}}$. Therefore,
\begin{align*}
\nabla H(y^{*}_{-k} + cD_{-k}) \cdot D_{-k} < D_{k} \sum_{i \neq k} G_{ki} < D_{k} \alpha_{k} < D_{k}
\end{align*}
Since $\sum_{i \neq k} G_{ki} = \alpha_{k}$ (by construction) and $\alpha_{k} < 1$ (by assumption). Therefore, $H(\overline{w}^{*}_{-k} + D_{-k}) < H(\overline{w}^{*}_{-k}) + D_{k} = \overline{w}^{*}_{k} + D_{k}$. This means that $(\overline{w}^{*} + D)$ cannot be a fixed point. Contradiction. There is at most one fixed point.
\end{proof}
% ------------------------------------------------------------- %




\textbf{Extended Proof of \Cref{prop:res wage exogeneous}}
Finally, we provide fuller working, including step-by-step calculations, for the first part of \Cref{prop:res wage exogeneous}. \textbf{Set-up:}
It follows from the preferences that if a worker accepts a wage $w_{i}$ then she gets a present value of
\begin{align*}
W(x) = \frac{f \left( w_{it} - R_{i}  \right) }{ 1 - \beta}
\end{align*}

\noindent We will suppress the $i$ subscripts for convenience. The expected value of searching one more time is
\begin{align*}
U = \beta \mathbb{E}[ \max \{ U , W(w') \} ]
\end{align*}

\noindent Let $V(x) = \max \{ U , W(w) \}$ be the value of having a job offer in hand.
\begin{align*}
V(w) = \max_{ \{a,r \} } \left\lbrace \frac{ f \left( w - R  \right) }{1 - \beta}  ,  \beta \mathbb{E}[ V(w')] \right\rbrace   \\
V(w) = \max_{ \{a,r \} } \left\lbrace \frac{ f \left( w - R  \right) }{1 - \beta}  ,  \beta \int_{0}^{Z} V(w') d G(w') \right\rbrace   \\
\end{align*}

\noindent \textbf{Solution:} first notice that the reservation wage solves
\begin{align*}
\frac{ f \left( \overline{w} - R  \right) }{1 - \beta}  &=  \beta \int_{0}^{Z} V(w') d G(w')
\intertext{Which we can rewrite as }
\frac{ f \left( \overline{w} - R  \right) }{1 - \beta}  &=  \beta \int_{0}^{\overline{w}} V(w') d G(w') + \beta \int_{\overline{w}}^{Z} V(w') d G(w')
\intertext{For any wage below the reservation wage, the offer gets rejected and the value function is the reservation wage earned for ever. For any wage above the reservation wage, the offer gets accepted and the value function is that wage earned for ever. }
\frac{ f \left( \overline{w} - R  \right) }{1 - \beta}  &=
		\beta \int_{0}^{\overline{w}} \frac{ f \left( \overline{w} - R  \right) }{1 - \beta} d G(w') 	+ \beta \int_{\overline{w}}^{Z} \frac{ f \left( w' - R  \right) }{1 - \beta} d G(w')
\intertext{We can split apart the LHS }
\frac{ f \left( \overline{w} - R  \right) }{1 - \beta} \int_{0}^{\overline{w}} d G(w') +
\frac{ f \left( \overline{w} - R  \right) }{1 - \beta} \int_{\overline{w}}^{Z} d G(w')  &=
		\beta \frac{ f \left( \overline{w} - R  \right) }{1 - \beta} \int_{0}^{\overline{w}} d G(x') + \beta \int_{\overline{w}}^{Z} \frac{ f \left( w' - R \right) }{1 - \beta}  d G(w')
\intertext{Some terms cancel}
f \left( \overline{w} - R \right) \int_{0}^{\overline{w}} d G(w') &=
 	 \beta \int_{\overline{w}}^{Z} \frac{ f \left( w' - R \right) }{1 - \beta} d G(w')
 	 - \frac{ f \left( \overline{w} - R \right) }{1 - \beta} \int_{\overline{w}}^{Z} d G(w')
\end{align*}
\begin{align*}
\intertext{A sneaky add and subtract }
f \left(\overline{w} - R \right) \int_{0}^{\overline{w}} d G(w') &=
 	 \beta \int_{\overline{w}}^{Z} \frac{ f \left( w' - R \right) }{1 - \beta} d G(w')
 	 - \frac{ f \left(\overline{w} - R \right) }{1 - \beta} \int_{y}^{Z} d G(w') \\
 	 & \qquad \qquad
 	 + f \left( \overline{w} - R \right) \int_{\overline{w}}^{Z} d G(w')
 	 - f \left( \overline{w} - R \right) \int_{\overline{w}}^{Z} d G(w')
\intertext{Cancelling some terms}
f \left( \overline{w} - R \right) &=
 	 \beta \int_{\overline{w}}^{Z} \frac{ f \left( w' - R \right) }{1 - \beta} d G(w')
 	 - \frac{ f \left( \overline{w} - R \right) }{1 - \beta} \int_{\overline{w}}^{Z} d G(w')
 	 + f \left( \overline{w} - R \right) \int_{\overline{w}}^{Z} d G(w')
\end{align*}
\noindent Therefore
\begin{align*}
f \left(\overline{w} - R \right) =
 	 \frac{ \beta }{ 1 - \beta } \int_{\overline{w}}^{Z}   [ f \left( w' - R \right) - f \left( \overline{w} - R \right) ] d G(w')
\end{align*}

==> I.proofs_of_claims.tex <==
Here, we formalise and prove several claims made in the main text.

\begin{rem}
The benefits of consumption in equilibrium are independent of the network. The total cost of consumption is linear in an agent's Bonacich centrality.
\end{rem}
\begin{quote}
\begin{proof}
In equilibrium an agent's First Order Condition must hold. That is: $f'(x_i^* - \alpha_i \sum_j G_{ij} x_j^*) - c = 0$. This means that $x_i^* - \alpha_i \sum_j G_{ij} x_j^* = f^{'-1}(c)$. So equilibrium utility simplifies to $u_i^* = f(f^{'-1}(c)) - c C_i^b f^{'-1}(c)$. The result clearly follows from the simplified expression for equilibrium utility.
\end{proof}
\end{quote}


% ADDENDUM TO PROPOSITION 2
\begin{rem}[The special case of \Cref{prop:cost}]
If $\lambda_1 < 1$ and $f(a) = a^{\gamma}$, then $u_i^*$ is strictly increasing in $c$ if and only if $C_i^b > \frac{1}{\gamma}$
\end{rem}
% PROOF OF REMARK IMMEDIATELY ABOVE
\begin{quote}
\begin{proof}
This acts as an addendum to the proof of \Cref{prop:cost}. In the special case where $f(\cdot)$. $f(c) = c^\gamma$, then $f'^{-1}(c) = F(c) = \left( \frac{\gamma}{c} \right)^{\frac{1}{1 - \gamma}} $. Therefore $F'(c) = \left( \frac{-1}{1 - \gamma} \right) \left( \frac{\gamma}{c^{\gamma - 2}} \right)^{\frac{1}{1 - \gamma}}$ and $F'(c) \cdot c = \left( \frac{-1}{1 - \gamma} \right) \left( \frac{\gamma}{c} \right)^{\frac{1}{1 - \gamma}}$. Substituting in these terms, and rearranging terms yields: $\frac{d u_i^*}{d c} > 0$ if and only if $C_i^b > \frac{1}{\gamma}$.
\end{proof}
\end{quote}


\begin{rem}
In equilibrium, labour market sorting is positive. That is: $c \geq 0.5$.
\end{rem}
\begin{quote}
\begin{proof}
From the proof to \Cref{prop:sorting}, we know that a skilled agent $i$ chooses to work at a high productivity firm if:
\begin{align}
	\frac{1}{\alpha_{2i}}  \geq \frac{[(x_{SH} - x_{UH}) + (x_{SL} - x_{UL})] \cdot c + (x_{UH} - x_{UL}) }{ (x_{SH} - x_{SL}) } .
\end{align}
We also know that $\alpha_{2i} < 1$, and that higher values of $\alpha_{2i}$ make her less inclined to work for the high productivity firm. So consider an agent $i$ where $\alpha_{2i} = 1$ (or is arbitrarily close). In this case, rearranging the equation above, and flipping the inequality sign to consider the condition under which she will choose to \emph{low} productivity firm, yields:
\begin{align}
    (1 - c) (x_{SH} - x_{UH}) < c (x_{SL} - x_{UL}).
\end{align}
When $(x_{SH} - x_{UH}) > (x_{SL} - x_{UL})$, as I assumed in the main text, we need $c > 0.5$ to satisfy this equation.
\end{proof}
\end{quote}

==> J.homophily.tex <==
We now examine one of the most ubiquitous features of social networks -- the tendency for people to be disproportionately connected to those who are similar to themselves. In the networks literature, this is called \emph{homophily}. We first show that in a simple setting with two groups who differ in terms of their cost parameter, stronger homophily increases inequality of both consumption and welfare.\footnote{In the Online Appendix, we show that the results are not affected if we instead consider homophily in terms of reference strengths -- this suggests that the network structure is able to amplify or dampen inequality regardless of the underlying factors that drive the inequality.  Allowing for heterogeneous costs yields little insight into the areas we have explored so far. For completeness, the Online Appendix shows the heterogeneous-cost analogues to the main results so far.} 
We then allow agents to create the network endogenously, and show that this leads to extremely high homophily.

Before proceeding, it is helpful to set out a formal definition of homophily. There are many definitions in the literature, but the \emph{homophily index} is a simple and effective measure.\footnote{See \cite{jackson2008}, \cite{pin2016networks} and \cite{mcpherson2001birds}, among others, for discussion of homophily.}

\begin{defn}[Homophily index: from \citet{currarini2009economic}]\label{defn: homophily}
The homophily index for agent $i$ is the proportion of total links that are with agents in the same group as her. For an agent $i$ in group $\mathbb{P}$:
\begin{align*}
\hat{H}_{i} = \sum_{j \in \mathbb{P}} g_{ij}
\end{align*}
\end{defn}

\textbf{Two group case.} There are two groups, $H,L$. $i \in H \iff c_{i} = c_{H}$ and $i \in L \iff c_{i} = c_{L}$, with $c_h > c_L$. Also assume that $\alpha_{i} = \alpha$ for all $i$. To separate out the effects of homophily \textit{per se} from the effects of the reference strengths (which we studied earlier), we focus on \textit{rerouteing} links, rather than just adding or deleting them. As with \Cref{prop:perturbation}, we will consider comparison shifts to help with tractability.

Additionally, we will only consider comparison shifts where between-group links are rerouted to become within-group links. This is because these are the cases where the homophily index (weakly) increases for all agents, and so are unambiguous. We call these cases a \emph{segregation}.

\begin{defn}[Segregation]\label{defn: segregation}
A comparison shift $D$ is a ``segregation'' if and only if $D_{ij} > 0 \implies i,j \in P$, and $D_{ij} < 0 \implies i \in P , j \in P^{c}$. Where $P$ is one group ($H$ or $L$), and $P^{c}$ is the other group.
\end{defn}

Finally, we need the following assumption to help with tractability and to focus on the interesting case where the agents with each level of the marginal cost variable are recognisably grouped together in the network. 

\begin{ass}\label{ass: inward looking}
Every agent is influenced more by every agent in their own group, than by any agent in the other group. Formally: for every agents $i$ in group $P$, $(I- G)^{-1}_{ij} > (I- G)^{-1}_{ik} \ \forall j \in P \ , \ \forall k \in P^{c}$
\end{ass}

This assumption means that agents initially make stronger social comparisons with those in their own group than those in the other group. Note that this is in global sense, rather than simply the direct links in the social network. This is in line with the empirical observation that most real-world social networks exhibit homophily \citep{jackson2008}. With this simplification in place, we can now say that any segregation of the network increases consumption more for low cost agents than it does for high cost agents.

\begin{prop}\label{prop:homophily inequality}
Suppose that $\alpha_i = \alpha$ for all $i$ and Assumption \ref{ass: inward looking} holds. Then for any segregation, and for all $i \in H$ and for all $j \in L$: (i) $\Delta x_i^* < \Delta x_j^*$, and (ii) $\Delta u_i^* > \Delta u_j^*$.
\end{prop}
% ------------------------------------------------------------- %
% PROVES THAT HOMOPHILY INCREASES ACTIONS BY MORE FOR LOW COST AGENTS THAN HIGH COST AGENTS
% ------------------------------------------------------------- %
\begin{quote}
\begin{proof}[\emph{\textbf{Proof of Proposition \ref{prop:homophily inequality}.}}]
First, show that if $\alpha_i = \alpha$ for all $i$ and Assumption \ref{ass: inward looking} holds, then $i \in H$ and $j \in L \implies C_i^{gen} < C_j^{gen}$.  It follows from \Cref{lem:f inverse} that $c_H > c_L \ \implies \ f^{'-1}(c_H) < f^{'-1}(c_L)$. So we can now write: $x_i^* = f^{'-1}(c_H) \sum_{k \in H} B_{ik} + f^{'-1}(c_L) \sum_{k \in L} B_{ik}$. It follows from \Cref{rem:mean field existence} that if $\alpha_i = \alpha$ for all $i$ then $\sum_{k} (I - G)^{-1} = \frac{1}{1 - \alpha}$, and it follows from Assumption \ref{ass: inward looking} that $\sum_{k \in H} B_{ik} > \sum_{k \in L} B_{ik}$ if and only if $i \in H$. Taking these together, we find that $C_i^{gen} < C_j^{gen}$ for all $i \in H$ and $j \in L$.

%Define some terms. Let $x_{i}^{*} =  \sum_{j} (I - G)^{-1}_{ij} f^{'-1}(c_{j}) = C^{gen}_{i}$ and $\tilde{x}_{i}^{*} = \sum_{j} (I - \tilde{G})^{-1}_{ij} f^{'-1}(c_{j})  = \tilde{C}^{gen}_{i}$. Then let $\Delta x_{i}^{*} \equiv  \tilde{x}_{i}^{*} - x^{*}_{i}$. \\

Now let $\Delta x_i^*$ be the change in $x^*$ due to a change in the network structure. From Proposition \ref{lem:perturb effect} (in fact, the generalised version, \Cref{prop:perturb effect restated}, in the Online Appendix), when an agent $r$ `reroutes' a link \textit{from} agent $d$ \textit{to} agent $u$.
\vspace{-4mm}
\begin{align*}
\Delta x_{i}^{*} = \frac{ \phi B_{ir} (C^{gen}_{u} - C^{gen}_{d})}{1 - \phi (B_{ur} - B_{dr}) }
\end{align*}
\noindent There are two ways in which a between-group link can be rerouted to a within-group link. First, an agent $r \in H$ reroutes a link from $d \in L$ to $u \in H$. Second, an agent $r \in L$ reroutes a link from $d \in H$ to $u \in L$. 

\noindent \textbf{Case 1:} since $u \in H$ and $d \in L$, then $(C^{gen}_{u} - C^{gen}_{d}) < 0$. Therefore $\Delta x_{i}^{*}  < 0$ (since $B_{ij} > 0 \ \forall i,j$). Further, $B_{ir} > B_{jr} \ \forall i \in H \ \forall j \in L$ by assumption \ref{ass: inward looking}, so  $\Delta x_{i}^{*} < \Delta x_{j}^{*} \ \forall i \in H \ \forall j \in L$. 

\noindent \textbf{Case 2:} since $u \in L$ and $d \in H$, then $(C^{gen}_{u} - C^{gen}_{d}) > 0$ by assumption. Therefore $\Delta x_{i}^{*}  > 0$ (since $B_{ij} > 0 \ \forall i,j$). Further, $B_{jr} > B_{ir} \ \forall i \in H \ \forall j \in L$ by assumption \ref{ass: inward looking}, so  $\Delta x_{i}^{*} < \Delta x_{j}^{*} \ \forall i \in H \ \forall j \in L$. \\

%\noindent In both cases we have $\Delta x_{i}^{*} > \Delta x_{j}^{*} \ \forall i \in H \ \forall j \in L$, which implies that $| \tilde{x}_{H}^{*} - \tilde{x}_{L}^{*} | > | x_{H}^{*} - x_{L}^{*} |$, where $x_{\mathcal{P}}^{*} = \frac{1}{\# \{ \mathcal{P} \} } \sum_{i \in \mathcal{P}} x_{i}^{*}$. Therefore group-level inequality rises.
\end{proof}
\end{quote}
% ------------------------------------------------------------- %

Where $\Delta$ denotes the change in the variable due to the segregation. The low cost agents start out with higher consumption (by \Cref{ass: inward looking}), so when an agent $j\in L$ segregates, she is now making comparisons with a higher consumption neighbour than before. This increases her reference point, and so increases her consumption and decreases her utility. Since the two groups are sufficiently inward-looking, the spillover effects are more concentrated within her group, so other low cost agents are more affected than the high cost ones. This logic applies all in reverse for a high cost agent.

The gap disparity in consumption between groups therefore rises. However, this higher inequality does not necessarily show up in the individual-level data commonly collected: overall variance or the Gini coefficient may fall following a segregation. This happens when the within-group inequality decreases, and this more than offsets the increase in between-group inequality. 

We face the same limitation as \Cref{prop:perturbation} here -- we can only consider very simple changes to the network structure. While the condition in \Cref{ass: inward looking} initially holds by assumption, we cannot guarantee that it holds after the segregation. Nevertheless, if segregations do not cause Assumption \ref{ass: inward looking} to be violated, then we can just apply Proposition \ref{prop:homophily inequality} repeatedly. Example 1 illustrates this intuition on a small network.

%This is due to the spillovers of low cost (i.e. high centrality) agents. Being more closely connected to a low cost agent increases an agent's consumption. With higher homophily, these positive spillovers are (increasingly) concentrated within the $H$ group, increasing the disparity between groups.

%It follows straightforwardly from \Cref{prop:homophily inequality} that the gap between average consumption of low cost and high cost agents increases following a segregation of the network. In this sense, homophily increases inequality. 

%\Cref{prop:homophily inequality} considers a change to the network structure (i.e. a matrix perturbation), so we face the same obstacle to achieving general results as in \Cref{prop:perturb effect}. We cannot extend Proposition \ref{prop:homophily inequality} to multiple small changes to the network structure as we cannot guarantee that Assumption \ref{ass: inward looking} will not be violated.\footnote{We \emph{assume} it holds before any change to the network, but it could be violated \emph{following} a small change.}  In spite of this, we might intuitively expect the logic to carry through to more than one segregation. Indeed, if perturbations do not cause Assumption \ref{ass: inward looking} to be violated, then we can apply Proposition \ref{prop:homophily inequality} repeatedly. The example below illustrates this intuition on a small network. \\

\newpage
\noindent \textbf{Example 1:}
In this example, we have heterogeneous reference strength and constant costs. $\alpha_{i} = 0.7$ for $i \in \{ A, B, C \}$, $\alpha_{i} = 0.6$ for $i \in \{ D, E, F \}$, $c = 0.1$, $f(z) = z^{0.5}$. Group H consists of nodes $A, B, C$ and group L consists of nodes $D, E, F$. Figure \ref{fig: example1} shows the initial network, and then reroutes each pair of between-group links in turn. It shows that in this case, consumption rises by more for the group H agents at each step.

% TIKZ PICTURE HERE: THE SEGREGATION EXAMPLE
\input{tikz_pictures/segregation_example}
\newpage

\noindent We now examine homophily in terms of the reference strengths, $\alpha_i$. That an analogous result to \Cref{prop:homophily inequality} holds suggests that it is homophily, and not something else, that is driving the inequality of outcomes.

Here, we partition the set of agents into two groups, $H$ and $L$. Now  $i \in H \iff \alpha_{i} = \alpha_{H}$ and $i \in L \iff \alpha_{i} = \alpha_{L}$, with $\alpha_{H} > \alpha_{L}$ and $c_{i} = c$ for all $i$. Before stating the analogy to \Cref{prop:homophily inequality}, we first need to show that optimal actions are higher in the high strength group. Note that when we define homophily in terms of costs, the high cost group has low actions -- whereas here, the high strength group has \emph{high} actions. Therefore the result will appear to be inverted. 

% HIGH STRENGTH GROUP HAS HIGHER ACTIONS UNDER INWARD LOOKING ASSUMPTION
\begin{rem}\label{homoph 3}
Suppose Assumption \ref{ass: inward looking} holds. Then $x^{*}_{i} > x^{*}_{j} \ \forall i \in H \ , \ \forall j \in L$ up to a third order approximation.
\end{rem}
% PROOF OF THE REMARK IMMEDIATELY ABOVE
\begin{quote}
\begin{proof}[\emph{\textbf{Proof of Remark \ref{homoph 3}.}}]
Take a third order approximation of agent $i$'s Bonacich centrality.
\begin{align*}
%%% B &= I + ag + (ag)^{2} + (ag)^{3} + ... \\
C^{b}_{i} &= \sum_{j} B_{ij} = \sum_{k=0}^{\infty} \sum_{j} (ag)^{k}_{ij} \approx 1 + \alpha_{i} + \sum_{j} (ag)^{2}_{ij} + \sum_{j} (ag)^{3}_{ij}
\end{align*}

Consider the second order term, noting that $\sum_j g_{sj} = 1$ and $\frac{1}{n} \sum_{s}  \alpha_{s} = \overline{\alpha}$:
\begin{align*}
\sum_{j} (ag)^{2}_{ij} &= \sum_{j} \sum_{s} \alpha_{i} g_{is} \alpha_{s} g_{sj} = \alpha_{i} ( \overline{\alpha} + \Cov( g_{is} , \alpha_{s} )  )
\end{align*}

Consider the third order term:
\begin{align*}
\sum_{j} (ag)^{3}_{ij} &= \sum_{j} \sum_{s} \alpha_{i} g_{is} (ag)^{2}_{sj} = \alpha_{i} \overline{\alpha} \sum_{s} g_{is} \alpha_{s}  + \alpha_{i} \sum_{s} g_{is} \alpha_{s} \Cov( g_{sk} , \alpha_{k} )
\intertext{Letting $\Cov( g_{sk} , \alpha_{k} ) = \chi_{s}$ }
&= \alpha_{i} \overline{\alpha} ( \overline{\alpha} + \Cov( g_{is} , \alpha_{s} )) +  \alpha_{i} \sum_{s} g_{is} \alpha_{s} \chi_{s} \\
&= \alpha_{i} \overline{\alpha} ( \overline{\alpha} + \Cov( g_{is} , \alpha_{s} )) + \alpha_{i} \left( \sum_{s} g_{is} \sum_{s} \alpha_{s} \chi_{s} + \Cov(g_{is}, \alpha_{s} \chi_{s}) \right) \\
&= \alpha_{i} \overline{\alpha} ( \overline{\alpha} + \Cov( g_{is} , \alpha_{s} )) + \alpha_{i} \left( \overline{\alpha} \ \overline{\chi} + \Cov(\alpha_{s} , \chi_{s}) +  \Cov(g_{is}, \alpha_{s} \chi_{s}) \right)
\end{align*}

\noindent This yields an approximation for Bonacich centrality:
\begin{align*}
C^{b}_{i} &\approx 1 + \alpha_{i} + \alpha_{i} (1 + \overline{\alpha})(\overline{\alpha} + \Cov( g_{is} , \alpha_{s} )  ) + \alpha_{i} \left( \overline{\alpha} \ \overline{\chi} + \Cov(\alpha_{s} , \chi_{s}) + \Cov(g_{is}, \alpha_{s} \chi_{s}) \right)
\end{align*}
It follows from the Assumption \ref{ass: inward looking} that agents are influenced more by those in their own group than those in the other group. This means that $\Cov(g_{is} , \alpha_{s}) = \chi_{i} > 0$ for all $i \in H$ and $\Cov(g_{is} , \alpha_{s}) = \chi_{i} < 0$ for all $i \in L$. It then follows that $\Cov(\alpha_{s}, \chi_{s}) > 0$ for all $s \in H$ and $\Cov(\alpha_{s}, \chi_{s}) < 0$ for all $s \in L$. This is because $\chi_{s}$ is positive when $\alpha_{s}$ is larger, and negative when $\alpha_{s}$ is small. This further implies that $\Cov(g_{is}, \alpha_{s} \chi_{s}) \ \forall i \in H$ and $\Cov(g_{is}, \alpha_{s} \chi_{s}) < 0 \ \forall i \in L$. This is by identical logic. This property of the covariance terms and the fact that $\alpha_{H} > \alpha_{L}$ implies that H-group agents have higher Bonacich centrality than L-group agents.
$C^{b}_{i} \gtrapprox C^{b}_{j} \quad \forall i \in H \ , \ \forall j \in L$. Therefore $x^{*}_{i} \gtrapprox x^{*}_{j}$ for all $i \in H$ and for all $j \in L$.
\end{proof}
\end{quote}

With this in place, we can now state the analogy to \Cref{prop:homophily inequality}.

\begin{rem}\label{homoph 5}
Suppose Assumption \ref{ass: inward looking} holds. Then for any network structure $g$, any segregation increases actions for every high-strength agent by more than for any low-strength agent. That is: $\Delta x_i > \Delta x_j$ for all $i \in H, j \in L$
\end{rem}
% PROOF OF REMARK IMMEDIATELY ABOVE
\begin{quote}
\begin{proof}[\emph{\textbf{Proof of Remark \ref{homoph 3}.}}]
From \Cref{homoph 3}, we have: $C^{b}_{i} \gtrapprox C^{b}_{j} \quad \forall i \in H \ , \ \forall j \in L$. Now let $\Delta x_i^*$ be the change in $x^*$ due to a change in the network structure. From \Cref{prop:perturb effect restated}, when an agent $r$ `reroutes' a link \textit{from} agent $d$ \textit{to} agent $u$
\begin{align*}
\Delta x_{i}^{*} = \frac{ \phi B_{ir} (C^{b}_{u} - C^{b}_{d}) f{'-1}(c) }{1 - \phi (B_{ur} - B_{dr}) }
\end{align*}
\noindent There are two ways in which a between-group link can be rerouted to a within-group link. First, an agent $r \in H$ reroutes a link from $d \in L$ to $u \in H$. Second, an agent $r \in L$ reroutes a link from $d \in H$ to $u \in L$. 

\noindent \textbf{Case 1:} since $u \in H$ and $d \in L$, then $(C^{b}_{u} - C^{b}_{d}) > 0$. Therefore $\Delta x_{i}^{*}  > 0$ (since $B_{ij} > 0 \ \forall i,j$). Further, $B_{ir} > B_{jr} \ \forall i \in H \ \forall j \in L$ by assumption \ref{ass: inward looking}, so  $\Delta x_{i}^{*} > \Delta x_{j}^{*} \ \forall i \in H \ \forall j \in L$. 

\noindent \textbf{Case 2:} since $u \in L$ and $d \in H$, then $(C^{b}_{u} - C^{b}_{d}) < 0$. Therefore $\Delta x_{i}^{*}  < 0$ (since $B_{ij} > 0 \ \forall i,j$). Further, $B_{ir} < B_{jr} \ \forall i \in H \ \forall j \in L$ by assumption \ref{ass: inward looking}, so  $\Delta x_{i}^{*} > \Delta x_{j}^{*} \ \forall i \in H \ \forall j \in L$. \\
\end{proof}
\end{quote}


==> Y.OA_intro.tex <==
This appendix contains additional material that supplements the main text. \Cref{extensions:K goods} shows that allowing $K$ different goods has no impact. This is due to the additive separability in preferences. \Cref{extensions:loss aversion} shows that adding loss aversion to the model has little impact. This is because agents are always able to consume above their reference point, and so need not experience losses. \Cref{extensions:network structure} sets out and proves a number of more technical results concerning the impact of comparison shifts to the network. These results formalise claims made shortly after \Cref{prop:perturbation}. 

\Cref{extensions:heterogeneous costs} shows that the main results from  \Cref{sec:results} are robust to introducing arbitrary heterogeneity in the cost parameter, $c$. It restates the main results from \Cref{sec:results} in this generalised setting, and shows that cost heterogeneity has little impact. \Cref{extensions: homophily} explores homophily, and links it to inequality of outcomes. Finally, \Cref{extension:claims} formalises and proves a number of claims made in the main text.

==> graphs/sorting_lemma_images.tex <==
\begin{figure}[h!]
     \centering
     \begin{subfigure}{0.3\textwidth}
        \centering
        \includegraphics[width=6cm]{graphs/sorting_lemma_A.PNG}
        \caption{An increase in $\alpha$ shifts the CDF $F(\alpha_2)$ to the right (red line to blue line in image).}
     \end{subfigure}
\hfill
     \begin{subfigure}{0.3\textwidth}
         \centering
        \includegraphics[width=6cm]{graphs/sorting_lemma_B.PNG}
        \caption{An increase in $\alpha$ shifts the CDF $F(h(c))$ to the left (red line to blue line in image).}
     \end{subfigure}
\hfill
     \begin{subfigure}{0.3\textwidth}
        \centering
       \includegraphics[width=6cm]{graphs/sorting_lemma_C.PNG}        
       \caption{A given shift in the CDF $F(h(c))$ causes a larger (in magnitude) fall in $c$ when the CDF is degenerate (the vertical line) than when it is not.}
     \end{subfigure}
\caption{Three simple graphs}\label{fig:three graphs}
\end{figure}


==> tikz_pictures/segregation_example.tex <==

\begin{figure}[H]
\centering
\caption{Segregation of a network}\label{fig: example1}
% NOTE: adjusting the multiple of textwidth adjusts the size of the whole image - choose this so that it fits on the page
\hspace{-3mm}
\begin{subfigure}[t]{0.5\textwidth}
\resizebox{8cm}{6cm}{ \fbox{
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=5cm,semithick]
  \tikzstyle{every state}=[fill=white, draw, text=black, circle]
  \node[state, label = {$x = 77.8$} ] 				(A)                	{$A$};
  \node[state, label =below right:{$x = 77.8$} ] 		(B) [below=2cm of A]  	{$B$};
  \node[state, label =below:{$x = 77.8$} ] 			(C) [below=2cm of B]  	{$C$};
  \node[state, label = {$x = 66.0$} ] 				(D) [right=3cm of A]  	{$D$};
  \node[state, label =above left:{$x = 66.0$} ] 		(E) [below=2cm of D]  	{$E$};
  \node[state, label =below:{$x = 66.0$} ] 			(F) [below=2cm of E]  	{$F$};

  \path (A)	edge [bend left=0, <->]			node {0.4} 			(B)
  			edge [bend right=50, <->]   		node[left] {0.4} 	(C)
  			edge [bend left=0, <->, green]		node {0.2}  		(D)
  		(B) edge [bend left=0, <->]			node {0.4}			(C)
  			edge [bend left=0, <->, blue]		node {0.2}			(E)
  		(C) edge [bend left=0, <->, red]		node {0.2}			(F)
  		(D)	edge [bend left=0, <->]			node {0.4}			(E)
  			edge [bend left=50, <->]			node {0.4}			(F)
  		(E) edge [bend left=0, <->]			node {0.4} 			(F);

\end{tikzpicture}  } }
\vspace{5mm}
\centering
\caption{Initial Network.}\label{fig: example1:a} %$x_{H} - x_{L} = 11.8$, $\Var(x_{i}) = 34.8$}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.5\textwidth}
\resizebox{8cm}{6cm}{ \fbox{
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=5cm,semithick]
  \tikzstyle{every state}=[fill=white, draw, text=black, circle]
  \node[state, label = {$x = 80.2$} ] 				(A)                	{$A$};
  \node[state, label =below right:{$x = 78.8$} ] 		(B) [below=2cm of A]  	{$B$};
  \node[state, label =below:{$x = 78.8$} ] 			(C) [below=2cm of B]  	{$C$};
  \node[state, label = {$x = 66.4$} ] 				(D) [right=3cm of A]  	{$D$};
  \node[state, label =above left:{$x = 66.3$} ] 		(E) [below=2cm of D]  	{$E$};
  \node[state, label =below:{$x = 66.3$} ] 			(F) [below=2cm of E]  	{$F$};

  \path (A)	edge [bend right=10, ->]		node[left] {0.5} 		(B)
  			edge [bend right=50, ->]   	node {0.5} 		(C)
  		(B) edge [bend right=10, ->]		node[right] {0.4}		(A)
  			edge [bend left=0, <->]		node {0.4}		(C)
  			edge [bend left=0, <->, blue]	node {0.2}		(E)
  		(C) edge [bend left=70, ->]		node {0.4}		(A)
  			edge [bend left=0, <->, red]	node {0.2}		(F)
  		(D)	edge [bend right=10, ->]		node[left] {0.5}		(E)
  			edge [bend left=50, ->]		node[left] {0.5}		(F)
  		(E) edge [bend right=10, ->]		node[right] {0.4} 		(D)
  			edge [bend left=0, <->]		node {0.4} 		(F)
  		(F) edge [bend right=70, ->]		node[right] {0.4}		(D);

\end{tikzpicture}  } }
\vspace{5mm}
\caption{Cut first pair of links.}\label{fig: example1:b} %$x_{H} - x_{L} = 12.9$, $\Var(x_{i}) = 41.7$}
\end{subfigure}
\end{figure}

\begin{figure}[H]\ContinuedFloat
\centering
%\caption{An Example Network, continued. }\label{fig: example1b}
% NOTE: adjusting the multiple of textwidth adjusts the size of the whole image - choose this so that it fits on the page
\hspace{-3mm}
\begin{subfigure}[t]{0.5\textwidth}
\resizebox{8cm}{6cm}{ \fbox{
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=5cm,semithick]
  \tikzstyle{every state}=[fill=white, draw, text=black, circle]
  \node[state, label = {$x = 81.4$} ] 				(A)                	{$A$};
  \node[state, label =below right:{$x = 81.4$} ] 		(B) [below=2cm of A]  	{$B$};
  \node[state, label =below:{$x = 79.7$} ] 			(C) [below=2cm of B]  	{$C$};
  \node[state, label = {$x = 63.6$} ] 				(D) [right=3cm of A]  	{$D$};
  \node[state, label =above left:{$x = 63.6$} ] 		(E) [below=2cm of D]  	{$E$};
  \node[state, label =below:{$x = 65.9$} ] 			(F) [below=2cm of E]  	{$F$};

  \path (A)	edge [bend left=0, <->]			node {0.5} 			(B)
  			edge [bend right=50, ->]   		node[right] {0.5} 	(C)
  		(B) edge [bend left=10, ->]			node {0.5}			(C)
  		(C) edge [bend left=70, ->]			node[left] {0.4}	(A)
  			edge [bend left=10, ->]			node {0.4} 			(B)
  			edge [bend left=0, <->, red]		node {0.2}			(F)
  		(D)	edge [bend left=0, <->]			node {0.5}			(E)
  			edge [bend left=50, ->]			node[left] {0.5}	(F)
  		(E) edge [bend left=10, ->]			node {0.5} 			(F)
  		(F)	edge [bend left=10, ->]			node {0.4}			(E)
  			edge [bend right=70, ->]			node[right] {0.4}	(D);
\end{tikzpicture}  } }
\caption{Cut second pair of links.}\label{fig: example1:c} %$x_{H} - x_{L} = 16.7$, $\Var(x_{i}) = 70.2$}
\end{subfigure}
\hfill
\centering
\begin{subfigure}[t]{0.5\textwidth}
\resizebox{8cm}{6cm}{ \fbox{
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=5cm,semithick]
  \tikzstyle{every state}=[fill=white, draw, text=black, circle]
  \node[state, label = {$x = 83.3$} ] 				(A)                	{$A$};
  \node[state, label =below right:{$x = 83.3$} ] 		(B) [below=2cm of A]  	{$B$};
  \node[state, label =below:{$x = 83.3$} ] 			(C) [below=2cm of B]  	{$C$};
  \node[state, label = {$x = 62.5$} ] 				(D) [right=3cm of A]  	{$D$};
  \node[state, label =above left:{$x = 62.5$} ] 		(E) [below=2cm of D]  	{$E$};
  \node[state, label =below:{$x = 62.5$} ] 			(F) [below=2cm of E]  	{$F$};

  \path (A)	edge [bend right=0, <->]		node[left] {0.5} 		(B)
  			edge [bend right=50, <->]   	node {0.5} 				(C)
  		(B) edge [bend left=0, <->]		node[left] {0.5}		(C)
  		(D)	edge [bend right=0, <->]		node[right] {0.5}		(E)
  			edge [bend left=50, <->]		node[left] {0.5}		(F)
  		(E) edge [bend left=0, <->]		node[right] {0.5} 		(F);
\end{tikzpicture}
} }
\caption{Cut third pair of links.}\label{fig: example1:d} % $x_{H} - x_{L} = 20.8$, $\Var(x_{i}) = 108.5$}
\end{subfigure}
\end{figure}

\begin{comment}
\begin{table}[H]
\centering
\begin{tabular}{llllll}
						& Fig 1(a) 	& half 		& Fig 1(b) 		& Fig 2(a) 	& Fig 2(b) \\
$x_{a}$ 				& 77.8302	& 80.1514	& 80.0238 		& 81.3649	& 83.3333        \\
$x_{b}$ 				& 77.8302	& 78.7877	& 78.6054    	& 81.3649 	& 83.3333        \\
$x_{c}$ 				& 77.8302	& 78.7877	& 78.6054  		& 79.6777	& 83.3333        \\
$x_{d}$ 				& 66.0377	& 66.4516	& 64.3825   	& 63.6122	& 62.5        \\
$x_{e}$ 				& 66.0377	& 66.3196	& 65.6374  		& 63.6122	& 62.5        \\
$x_{f}$ 				& 66.0377	& 66.3196	& 65.6374  		& 65.0952	& 62.5        \\
$\Var(x_{i})$ 			& 34.765486 & 41.673476 & 48.412752 	& 70.2493	& 108.506944  \\
$| x_{H} - x_{L} |$	& 11.7925	& 12.8787	& 13.8591   	& 16.6959	& 20.8333
\end{tabular}
\end{table}
\end{comment}

==> tikz_pictures/sortin_lemma_separated.tex <==
%\DeclareMathOperator{\CDF}{cdf}
\def\cdf(#1)(#2)(#3){0.5*(1+(erf((#1-#2)/(#3*sqrt(2)))))}%
\newcommand{\pw}{16cm}
\newcommand{\lw}{5pt}


% F1
\begin{figure}
    \centering
        \begin{tikzpicture}[font=\Huge]
            \begin{axis}[width=\pw, xlabel=$\alpha_2$, xmajorticks=false, xlabel near ticks,  
                        ylabel=$F(\alpha_2)$, ytick={0,1}, ylabel near ticks, grid=none, font=\huge]
            \addplot[smooth, line width =\lw, red]  gnuplot{\cdf(x)(0)(1)};
            \addplot[smooth, line width =\lw, blue] gnuplot{\cdf(x)(1)(1)};
            \end{axis}
        \end{tikzpicture}
\end{figure}

%F2
\begin{figure}
    \centering
        \begin{tikzpicture}[font=\Huge]
            \begin{axis}[width=\pw, xlabel=$c$, xmajorticks=false, xlabel near ticks,  
                        ylabel=$F(h(c))$, ymajorticks=false, ylabel near ticks,  grid=none]
            \addplot[smooth, line width =\lw, blue]    gnuplot{1 - \cdf(x)(0)(1)};
            \addplot[smooth, line width =\lw, red]     gnuplot{1 - \cdf(x)(1)(1)};
            \addplot[smooth, line width =\lw, black] gnuplot{(0.1)*x + 0.5};
            \end{axis}
        \end{tikzpicture}
\end{figure}

% F3
\begin{figure}
    \centering
        \begin{tikzpicture}[font=\Huge]
            \begin{axis}[width=\pw, xlabel=$c$, xmajorticks=false, xlabel near ticks,
                        ylabel=$F(h(c))$, ymajorticks=false, ylabel near ticks, grid=none]
            \addplot[smooth, line width =\lw, blue]    gnuplot{1 - \cdf(x)(0)(1)};
            \addplot[smooth, line width =\lw, red]     gnuplot{1 - \cdf(x)(1)(1)};
            \addplot[smooth, line width =\lw, black] gnuplot{(0.1)*x + 0.5};
            \addplot[smooth, line width =\lw, green]   gnuplot{x=0};
            \addplot[smooth, line width =\lw, magenta] coordinates {(0.85,0)(0.85,1)};
            \addplot[smooth, line width =\lw, green] coordinates {(-0.15,0)(-0.15,1)};
            \end{axis}
        \end{tikzpicture}
\end{figure}


==> tikz_pictures/sorting_lemma_graphs.tex <==
%\DeclareMathOperator{\CDF}{cdf}
\def\cdf(#1)(#2)(#3){0.5*(1+(erf((#1-#2)/(#3*sqrt(2)))))}%
\newcommand{\pw}{6cm}
\newcommand{\lw}{1.5pt}

\begin{figure}[h!]
     \centering
     \begin{subfigure}[h]{0.3\textwidth}
        \centering
        \begin{tikzpicture}
            \begin{axis}[width=\pw, xlabel=$\alpha_2$, xmajorticks=false, xlabel near ticks,  
                        ylabel=$F(\alpha_2)$, ytick={0,1}, ylabel near ticks, grid=none]
            \addplot[smooth, line width =\lw, red]  gnuplot{\cdf(x)(0)(1)};
            \addplot[smooth, line width =\lw, blue] gnuplot{\cdf(x)(1)(1)};
            \end{axis}
        \end{tikzpicture}
        \caption{An increase in $\alpha$ shifts the CDF $F(\alpha_2)$ to the right (red line to blue line in image).}
     \end{subfigure}
\hfill
     \begin{subfigure}[h]{0.3\textwidth}
         \centering
        \begin{tikzpicture}
            \begin{axis}[width=\pw, xlabel=$c$, xmajorticks=false, xlabel near ticks,  
                        ylabel=$F(h(c))$, ymajorticks=false, ylabel near ticks,  grid=none]
            \addplot[smooth, line width =\lw, blue]    gnuplot{1 - \cdf(x)(0)(1)};
            \addplot[smooth, line width =\lw, red]     gnuplot{1 - \cdf(x)(1)(1)};
            \addplot[smooth, line width =\lw, black] gnuplot{(0.1)*x + 0.5};
            \end{axis}
        \end{tikzpicture}
        \caption{An increase in $\alpha$ shifts the CDF $F(h(c))$ to the left (red line to blue line in image).}
     \end{subfigure}
\hfill
     \begin{subfigure}[h]{0.3\textwidth}
         \centering
        \begin{tikzpicture}
            \begin{axis}[width=\pw, xlabel=$c$, xmajorticks=false, xlabel near ticks,
                        ylabel=$F(h(c))$, ymajorticks=false, ylabel near ticks, grid=none]
            \addplot[smooth, line width =\lw, blue]    gnuplot{1 - \cdf(x)(0)(1)};
            \addplot[smooth, line width =\lw, red]     gnuplot{1 - \cdf(x)(1)(1)};
            \addplot[smooth, line width =\lw, black] gnuplot{(0.1)*x + 0.5};
            \addplot[smooth, line width =\lw, green]   gnuplot{x=0};
            \addplot[smooth, line width =\lw, magenta] coordinates {(0.85,0)(0.85,1)};
            \addplot[smooth, line width =\lw, green] coordinates {(-0.15,0)(-0.15,1)};
            \end{axis}
        \end{tikzpicture}
        \caption{A given shift in the CDF $F(h(c))$ causes a larger (in magnitude) fall in $c$ when the CDF is degenerate (the vertical line) than when it is not.}
     \end{subfigure}
\caption{Three simple graphs}\label{fig:three graphs}
\end{figure}



\begin{comment}
\begin{figure}
\centering
%\includegraphics{}
\caption{An increase in $\alpha$ shifts the CDF $F(\alpha_2)$ to the right (red line to blue line in image).}\label{fig:my_label}
    \begin{tikzpicture}
        \begin{axis}[xlabel=$\alpha_2$,xmajorticks=false, ylabel=$F(\alpha_2)$, ytick={0,1}, grid=none]
        \addplot[smooth, line width = 3pt, red] gnuplot{\cdf(x)(0)(1)};
        \addplot[smooth, line width = 3pt, blue]gnuplot{\cdf(x)(1)(1)};
        %\addplot[smooth,green]gnuplot{\cdf(x)(1)(1)};
        %\addplot[smooth,orange]gnuplot{\cdf(x)(2)(1)};
        \end{axis}
    \end{tikzpicture}
\end{figure}

\end{comment}
